Rethinking the Relationship between Recurrent and Non-Recurrent Neural Networks: A Study in Sparsity

Neural networks (NN) can be divided into two broad categories, recurrent and non-recurrent. Both types of neural networks are popular and extensively studied, but they are often treated as distinct families of machine learning algorithms. In this position paper, we argue that there is a closer relationship between these two types of neural networks than is normally appreciated. We show that many common neural network models, such as Recurrent Neural Networks (RNN), Multi-Layer Perceptrons (MLP), and even deep multi-layer transformers, can all be represented as iterative maps. The close relationship between RNNs and other types of NNs should not be surprising. In particular, RNNs are known to be Turing complete, and therefore capable of representing any computable function (such as any other types of NNs), but herein we argue that the relationship runs deeper and is more practical than this. For example, RNNs are often thought to be more difficult to train than other types of NNs, with RNNs being plagued by issues such as vanishing or exploding gradients. However, as we demonstrate in this paper, MLPs, RNNs, and many other NNs lie on a continuum, and this perspective leads to several insights that illuminate both theoretical and practical aspects of NNs.

==> sections/Additional_iterations.tex <==
\section{Additional Iterations} \label{sec:additional-iterations}

\subsection{RNN with additional iterations}\label{sec:RNN-additional-iterations}
\subsubsection{Finite impulse response}

%In \S \ref{sec:RNN-block-iterative} it is important to recognize that the \eqref{eq:RNN-iterative-matrix-T} starting with initial conditions \eqref{eq:RNN-iterative-initial-condition-T} must be iterated $T$ times to achieve the equivalent outcome as \eqref{eq:RNN-defn}. Further iterations lead to undesirable results as shown below.

Applying the map $M_{RNN}$ one additional time reveals 
\begin{equation} \label{eq:RNN-iteration-4}
\begin{aligned}
    M \circ 
    M \circ 
    M \circ 
    M \circ 
    \begin{bmatrix}
        \mv{h}_0 \\
        0 \\
        0 \\
        0 \\
    \end{bmatrix} 
    &=       
    \begin{bmatrix}
        0                             & 0                             & 0                             & 0 \\
        \Wg{f_\theta(\cdot,\mv{x}_1)} & 0                             & 0                             & 0 \\
        0                             & \Wg{f_\theta(\cdot,\mv{x}_2)} & 0                             & 0 \\
        0                             & 0                             & \Wg{f_\theta(\cdot,\mv{x}_3)} & 0 \\
    \end{bmatrix}
    \circ 
    \begin{bmatrix}
        0 \\
        \Wg{f_\theta(0,\mv{x}_1)} \\
        \Wg{f_\theta \big( f_\theta(0,\mv{x}_1) ,\mv{x}_2 \big)} \\
        \Wg{f_\theta \Big(  f_\theta \big( f_\theta(\mv{h}_0,\mv{x}_1),\mv{x}_2 \big),\mv{x}_3} \Big)  \\
    \end{bmatrix} \\
    &=
    \begin{bmatrix}
        0 \\
        \Wg{f_\theta(0,\mv{x}_1)} \\
        \Wg{f_\theta \big( f_\theta(0,\mv{x}_1) ,\mv{x}_2 \big)} \\
        \Wg{f_\theta \Big(  f_\theta \big( f_\theta(0,\mv{x}_1),\mv{x}_2 \big),\mv{x}_3} \Big)  \\
    \end{bmatrix}
\end{aligned}
\end{equation}
which is independent of the input $\mv{h}_0$.

\subsubsection{Fixed point} \label{sec:RNN-fixed-point}
An additional application of $M_{RNN}$ 
\begin{equation} \label{eq:RNN_fixed_point}
\begin{aligned}
    M \circ 
    M \circ 
    M \circ 
    M \circ 
    M \circ
    \begin{bmatrix}
        \mv{h}_0 \\
        0 \\
        0 \\
        0 \\
    \end{bmatrix} 
    &=
    \begin{bmatrix}
        0                             & 0                             & 0                             & 0 \\
        \Wg{f_\theta(\cdot,\mv{x}_1)} & 0                             & 0                             & 0 \\
        0                             & \Wg{f_\theta(\cdot,\mv{x}_2)} & 0                             & 0 \\
        0                             & 0                             & \Wg{f_\theta(\cdot,\mv{x}_3)} & 0 \\
    \end{bmatrix}
    \circ 
    \begin{bmatrix}
        0 \\
        \Wg{f_\theta(0,\mv{x}_1)} \\
        \Wg{f_\theta \big( f_\theta(0,\mv{x}_1) ,\mv{x}_2 \big)} \\
        \Wg{f_\theta \Big(  f_\theta \big( f_\theta(0,\mv{x}_1),\mv{x}_2 \big),\mv{x}_3} \Big)  \\
    \end{bmatrix} \\ 
    &=
 \begin{bmatrix}
        0 \\
        \Wg{f_\theta(0,\mv{x}_1)} \\
        \Wg{f_\theta \big( f_\theta(0,\mv{x}_1) ,\mv{x}_2 \big)} \\
        \Wg{f_\theta \Big(  f_\theta \big( f_\theta(0,\mv{x}_1),\mv{x}_2 \big),\mv{x}_3} \Big)  \\
    \end{bmatrix}
\end{aligned}
\end{equation}
which in addition, shows that 
\begin{equation} \label{eq:MLP_fixed_point}
\begin{bmatrix}
        0 \\
        \Wg{f_\theta(0,\mv{x}_1)} \\
        \Wg{f_\theta \big( f_\theta(0,\mv{x}_1) ,\mv{x}_2 \big)} \\
        \Wg{f_\theta \Big(  f_\theta \big( f_\theta(0,\mv{x}_1),\mv{x}_2 \big),\mv{x}_3} \Big)  \\
    \end{bmatrix}  
\end{equation}
is a fixed point. 




==> sections/Continuation.tex <==
\section{Continuation paths to novel neural networks} \label{sec:continuation}

\subsection{Sequential2D} \label{sec:sequential2D}
\todo{This section needs to be cleaned up.  There are twp versions of the same thing.  Use the colored one, but keep the points from the earlier one.}
\begin{definition} \label{defn:seqential2D}
Sequential2D is a rectangular block matrix function within which each entry is a matrix function. A Sequential2D map is of the form
\begin{equation} \label{eq:Sequential2D}
    M = \begin{bmatrix} D_{11} &A_{12}  &\hdots &A_{1n}  \\
                        A_{21} &D_{22} &\hdots &A_{2n}  \\
                        \vdots &       &\ddots &\vdots \\
                        A_{n1} &A_{n2} &\hdots &D_{nn}
        \end{bmatrix}                    
\end{equation}
where at least one of $A_{ij}, i \not= j$ is non-zero.
By contrast Sequential1D maps are a subset of Sequential2D maps of the form
\begin{equation} \label{eq:Sequential1D}
    M = \begin{bmatrix} D_{11} &0      &\hdots  &0  \\
                        D_{22} &0      &\hdots  &0  \\
                        \vdots &\vdots &\ddots  &\vdots \\
                        D_{nn} &0      &\hdots  &0
        \end{bmatrix}                    
\end{equation}

\end{definition}
In many ways, \eqref{eq:Sequential2D} is a straightforward generalization of a block-defined matrix.  In particular, if every function $A_{ij}$ happened to be linear (i.e., a matrix) and the function composition operator $\circ$ were replaced with the dot-product, then \eqref{eq:Sequential2D} would be precisely a block defined matrix. 

\label{sec:generalizations}
This opens an entire range of new possibilities when considering a block iterative function of the form

% Full matrix
\begin{equation} \label{eq:generalizations-full}
    \begin{bmatrix}
        \Wy{W_{1,1}} & \Wr{W_{1,2}}  & \Wr{W_{1,3}}  & \Wr{W_{1,4}}  & \Wr{W_{1,5}} \\
        \Wg{W_{2,1}} & \Wy{W_{2,2}}  & \Wr{W_{2,3}}  & \Wr{W_{2,4}}  & \Wr{W_{2,5}} \\
        \Wb{W_{3,1}} & \Wg{W_{3,2}}  & \Wy{W_{3,3}}  & \Wr{W_{3,4}}  & \Wr{W_{3,5}} \\
        \Wb{W_{4,1}} & \Wb{W_{4,2}}  & \Wg{W_{4,3}}  & \Wy{W_{4,4}}  & \Wr{W_{4,5}} \\
        \Wb{W_{5,1}} & \Wb{W_{5,2}}  & \Wb{W_{5,3}}  & \Wg{W_{5,4}}  & \Wy{W_{5,5}} \\
    \end{bmatrix}
\end{equation}

In this notation, 
\begin{itemize}
\item $\Wg{W_{i+1,i}}$ corresponds to a standard MLP or, more generally, an NN that can be implemented as a Pytorch or Keras Sequential container.
\item $\Wb{W_{i+k,i}}, \; k>1$ corresponds to skip connections and finite impulse response (FIR) filters.
%\item We began the exploration of $\Wy{W_{i,i}}$ with the introduction of the $I$ in \eqref{FIXME} corresponds infinite impulse response filters.
%\item What do $\Wr{W_{i,j}}, \; j>i$ correspond to?  They are actually \emph{feedback} connections which also lead to infinite impulse response filters and classic RNNs.
\end{itemize}







==> sections/old/0ParkingLot.tex <==
NOTES from 7-6-2023 meeting:

Simon wants to work on the theory of computing the gradients with an eye towards understanding the geometry of the gradients.

We discussed $f(Ax)$ with regards to energy based methods and contrastive learning.  Note that $Ax$ fixes the dimension of a subpace, and $f$ allows this fixed dimension subspace to be a fixed dimension manifold.

Randy will work on the paper for the next few weeks.  In particular, move "red" stuff up and make simplier.  Other things Randy wants to do.

Note, MLPs with one off-diagonal entry are interesting.  They are not MLPs is any way!  But, they are within epsilon numerically of an MLP, and we show that they 
train the same.

Pytorch is an efficient implementation of automatic differentiation.  Also where the linear algebra happens on GPUs.

Doing and optimization with the constraint that $S$ is fixed.   

\todo{Talk about finite and infinite impulse response.  This is a red herring!  Especially with a finite number of iterations.}
\todo{Some vectors have finite impulse if they lay in the null-space of some vector,but other might have infinite impulse if they don't lay in the null-space}
\todo{We define a NN to be recurrent if there are *any* vectors that have infinite impulse.  I.e., applying the matrix and infinite number of times does not lead to a zero vector}


\subsection{Generalizations of the iterative RNN}


Starting from the RNN in (\ref{eq:affine}), we can derive a variety of other models by making different choices for the weight matrices $W_x$ and $W_h$.  In particular, one can simplify (\ref{eq:affine}) into a linear iterative equation by setting the activation function to the identity map $\sigma(x)=x$ and the bias vector to zero $b=0$.  This simplification allows us to rewrite (\ref{eq:affine}) as the following \emph{block sparse} matrix equation.

\begin{equation}
    \begin{bmatrix}
        0 & 0 \\
        W_x & W_h \\
    \end{bmatrix}
    \cdot
    \begin{bmatrix}
        x_t \\
        h_{t-1} \\
    \end{bmatrix}
    =
    \begin{bmatrix}
        0 \\
        W_x x_t + W_h h_{t-1} \\
    \end{bmatrix}.
    \label{eq:blockwise}
\end{equation}

The Recurrent Neural Network (RNN) \cite{rumelhart1986learning, Sherstinsky_2020} architecture was developed to overcome the limitations of MLP networks with respect to sequential data sets.  The RNN achieves this by iteratively applying shared parameters over each item in a sequence and incorporating a stored hidden state $H$ as outlined in \ref{eqn:Rnneq}.  Notation follows the mechanisms from equations \ref{eqn:layerw}, \ref{eqn:xmatrix}, \ref{eqn:wmatrix}.  The first hidden state is generally but not necessarily initialized as a zero matrix for $H_0$.  For each item in an input item $X_t$, a weight matrix $W$ is multiplied by $X_t$ at step $t$ while another weight matrix $W_{h}$ is multiplied by the hidden state $H_{t-1}$ from the previous step $t-1$ with some nonlinearity function (often a ReLU or tanh function) to the output.  The resulting output $H_t$ then serves as the next hidden state alongside the next item in the sequence $X_{t+1}$ using the same weight matrices $W_{h}$ and $W$, respectively.  When the last step in the sequence has been reached, the final hidden state serves as the output.

\begin{equation}\label{eqn:Rnneq}
    H_t=ReLU(W \cdot X_t+ W_{h} \cdot H_{t-1})
\end{equation}
\todo{Is the ReLU in the right place? --(Harsh) Yes (generally its tanh)}

By concatenated both weight matrices $W_{h}$ and $W$ as simply $W$ 
\begin{equation}
    W = \begin{bmatrix} W & W_h \\ \end{bmatrix},
\end{equation}

\noindent and concatenating $X_t$ and $H_{t-1}$ as a single input matrix ${Z}_{t}$,

\begin{equation}
    Z_t = \begin{bmatrix} X_t \\ H_{t-1} \\ \end{bmatrix}.
\end{equation}

The resulting RNN diagram is illustrated in Fig. \ref{fig:rnndiag}.  Through the use of shared weights, the RNN appears to unroll across the 
sequence steps with no theoretical limitation on sequence length paired with the ability to process varying length sequences.  The simple representation we've discussed portrays the RNN as a single-layer network processing data in a single direction moving forward through the sequence, however, in practice, they may be built as a series of recurrent layers feeding one another sequentially or processing data series bidirectionally.  Despite the technical ability for use with extremely long input data sequences, empirically, the performance has not been promising \cite{pmlr-v28-pascanu13, Sherstinsky_2020_rnn}. While backpropagating the errors over many iterations RNNs are known to become prone to either exploding or vanishing gradients that limit the network's memory over long sequences \cite{pmlr-v28-pascanu13}.  In these cases, the process of calculating gradients for repeated operations and nonlinearity functions across many steps may cause the magnitude of the gradient to either vanish or explode causing instability.  These effects are reduced through the use of ReLU as the choice of nonlinearity function, given that for positive values the gradient is unchanged.  Nonetheless, these general limitations inspired the creation of long short-term memory networks covered in Section \ref{sec:method_lstm}.

\begin{figure}[htbp]
     \centering
     \includegraphics[width=0.5\textwidth]{Figures/rnn.png}
     \caption{RNN diagram across steps of a sequence.}
     \label{fig:rnndiag}
\end{figure}





\subsubsection{General Theory} \label{sec:general_theory}

\begin{lemma}
For any affine operator $f(x) = W \cdot x + b$ there exists a linear operator 
$$
g(z) = 
\begin{bmatrix}
W & b \\
0 & 1 \\
\end{bmatrix}
\cdot
\begin{bmatrix}
x \\
1 \\
\end{bmatrix}
$$ 

such that 

$$
f(x) = proj_{\Omega_x}\left( g\left(\begin{bmatrix} x \\ 1 \end{bmatrix}\right) \right)
$$
\todo{clean up and cite}
\end{lemma}

\begin{theorem}
Let $\sigma_n(W_n \cdot \sigma_{n-1}( \hdots \sigma_2(W_2 \cdot \sigma_1(W_1 \cdot x))))$ be a set of nested functions
with $W_i \in \mathbb{R}_{d_i,d_{i-1}}$

Then, there exists an iterated function $g(z)$ where $g : \mathbb{R}_{d_0 + \hdots + d_n} \rightarrow \mathbb{R}_{d_0 + \hdots + d_n}$ written as

$$
\begin{bmatrix}
0      & 0      & \hdots & 0      & 0      \\
W_1    & 0      & \hdots & 0      & 0      \\
0      & W_2    & \hdots & 0      & 0      \\
\vdots & \vdots & \ddots & \vdots & \vdots \\
0      & 0      & \hdots & W_n    & 0      \\
\end{bmatrix}
$$

such that

$$
\begin{bmatrix}
0      & 0      & \hdots & 0      & 0      \\
W_1    & 0      & \hdots & 0      & 0      \\
0      & W_2    & \hdots & 0      & 0      \\
\vdots & \vdots & \ddots & \vdots & \vdots \\
0      & 0      & \hdots & W_n    & 0      \\
\end{bmatrix}
\cdot
\hdots
\cdot
\begin{bmatrix}
h_0 = x \\
h_1     \\
h_2     \\
\vdots  \\
h_n=y   \\
\end{bmatrix}
$$

\todo{notation not quite right.  Needs $\sigma \circ$}


\end{theorem}

\begin{theorem}
Let 

$$
\begin{bmatrix}
f_{0,0} & f_{0,1} \\
f_{1,0} & f_{1,1} \\
\end{bmatrix}
\circ
\begin{bmatrix}
x \\
y \\
\end{bmatrix}
=
\begin{bmatrix}
f_{0,0}(x) + f_{0,1}(y) \\
f_{1,0}(x) + f_{1,1}(y) \\
\end{bmatrix}
$$

then TBD
\todo{Theorem above needs something like this}
\end{theorem}


% aligned with an alternate set of recommended metrics.

% Our work first demonstrates the equivalence between RNN architectures represented as \emph{iterative functions}, where a single fixed function is iterated multiple times, and the typical feed-forward network's nested representation, where the various layer's outputs provide the inputs for the next, often differently shaped, layer.  These findings are then explored with the goal of more deeply understanding the drivers behind model performance.  Using MNIST-derived data sets to construct experiments, model performance is benchmarked both against other popular model architectures and against various configurations of RNN's.  Early rounds of experiments generate surprising results running contrary to common wisdom.  For instance, randomly arranged parameters within a sparse matrix demonstrate no distinguishable difference in model performance over the use of neatly arranged layers.  The findings seem to imply the specification of model structure through the number and dimension of layers is an artificial construct carrying little direct impact on the problems we study which attempts to indirectly approximate other implied model characteristics.  Sparsely arranged RNNs perform well across widely varied experiments when benchmarked against popular classes of competing model architectures. We demonstrate the benefit of sparsity and the inherent flexibility in the efficient allocation of weights in RNNs and when cast in the light of our suggested hyperparameterization, RNNs consistently outperformed or matched competing peer LSTM and MLP networks across a variety of tasks.

% The combination of these findings redirects the understanding of neural network architecture and hyperparameter selection towards a more universal approach while recommending alternative metrics for use in characterizing network structure.  These findings run counter to common intuition and open a path for further research into the implications of generalized architectures and randomly assigned sparse weight spaces toward model behavior.  Several characteristics such as model depth and model sparsity are presented which significantly improve the stability and expressiveness of model performance across a wider array of hyperparameters and reduce or eliminate performance differentials at significantly reduced parameter counts.  The aspect ratio of the weight space, reflecting the relationship between the depth and width of the weight space is introduced as a central feature governing model performance with direct ties to the iterative nature of RNNs.

% Sparse RNN's are shown to exhibit increased performance and training stability across a wider array of conditions and with reduced parameterization.  At its core, this approach allows comparable model performance with total trainable parameters reduced by more than a full order of magnitude in some cases while maintaining the ability to represent complex functions.  These findings echo similar findings from recent research.  Sparsity has been presented as a technique to reduce computational and memory needs for neural networks, while increasing ease of deployment across devices \cite{DBLP:journals/corr/abs-1711-02782}.  Commonly utilized methods involve either explicit block pruning methods or lasso regularization \cite{DBLP:journals/corr/abs-1711-02782, https://doi.org/10.48550/arxiv.1909.03011} applied through training with findings showing ranges from 80\% to more than 90\% sparsity resulting in minimal loss of accuracy.  Recent research has also shown that contrary to general belief the approach of training sparse RNNs from scratch may generate clear performance advantages over dense networks \cite{Liu2021}.  As a result, aside from solely improving parameterization efficiency, this approach has been demonstrated to be well-suited for complex systems with unknown dynamics such as hurricane topography \cite{10.1145/2908812.2908834}.

% While recurrent neural networks are widely understood to be iterative network architectures, the recognition that MLPs exist as a subset of RNNs carries secondary implications. \todo{While not detailed in this paper, we observe that our thought process in this work is driven by our desire to connect neural networks to dynamical systems...} By extending the generalized iterative approach to the wider body of neural network architectures there are opportunities for knowledge transfer from neighboring domains.  For example, such iterative equations are a central component of dynamic systems theory, a well-established field of study suited to complex systems often associated with feedback mechanisms and other nonlinear behavior.  These systems commonly feature sequentially dependent states, each evolved within a closed system such that knowledge of an initial state allows prediction of states at any subsequent point in time as is often encountered within classical physics.   Of course, we are not the first to appreciate the connection between RNNs and dynamic systems.  In particular, classic tools in dynamical systems, such as Lyapunov Exponents \cite{vogt2022lyapunov} and Koopman Operators \cite{dogra2020optimizing, yeung2019learning} have been used to understand neural networks. Perhaps the most famous example of the beauty and power of dynamical systems is the Mandelbrot Set which joins dynamical systems with fractal geometry \cite{10.2307/1721427}. Within the field of dynamical systems, those systems with \emph{sensitive dependence on initial conditions}, where small changes to the initial state may result in wildly varying outcomes or similarly chaotic behavior, share many commonalities with neural networks including feedback loops, interconnections, emergent patterns, and self-regulatory behavior which often emerge in the functions of neural networks \cite{DBLP:journals/corr/abs-1712-05577, REHMER20201243}. Such topics from dynamical systems provide a wide surface area for exploration and our motivation for much of our research in this area seeks to bridge the understanding between these dynamical systems. Of course, the current text only scratches the surface for results bridging these two fields, and additional directions for research will be discussed in Section \ref{sec:conclusions}




% \subsection{Traditional MLPs}

% Neural networks such as the traditional feed-forward multilayer perceptron \cite{MURTAGH1991183} architecture can be defined as a set of nested functions.  In this representation, each layer $i$ of the network and accompanying nonlinear activation function \cite{9108717} is represented as a function 

% \begin{equation}\label{eqn:layerw}
% f_i(\mathbf{h}_i) = \sigma(A_i \cdot \mathbf{h}_i + \mathbf{b}),
% \end{equation}

% \noindent with $A_i \in \mathbb{R}_{d_{i} \times d_{i-1}}$, $\mathbf{h}_i \in \mathbb{R}_{d_{i-1} \times 1}$, and $\mathbf{b} \in \mathbb{R}_{d_{i} \times 1}$. In particular, the affine function $W_i \cdot \mathbf{z} + \mathbf{b}$ of each layer if feed through a nonlinear activation function $\sigma$.  Each $f_i$ is then thought of as a \emph{layer} of the neural network, and in the MLP case, such an $f_i$ is called a \emph{dense layer} based on the density of the non-zero entries in the matrix $A_i$.

% The output of each function $f_i$ then forms the hidden layer input $\mathbf{h}$ of the subsequent function with the exception of the final layer of weights which provides model output $\mathbf{y}$.  The example provided in (\ref{eqn:nestedfx}) represents a typical four-layer network, 

% \begin{equation}\label{eqn:nestedfx}
%     \mathbf{y} = f_4(f_3(f_2(f_1(\mathbf{x})))),
% \end{equation}

% \noindent with $\mathbf{h}_0 = x$ being the input data for the MLP and $\mathbf{h}_4 = y$ being the MLP's output.

% Note, in the sequel we will often wish to emphasize the iterative and compositional nature of the function nesting in (\ref{eqn:nestedfx}), so we will denote the composition of two functions $f$ and $g$ using standard notation as $f(g(x)) = f \circ g(\mathbf{x})$.

% \begin{equation}\label{eqn:nestedf}
%     \mathbf{y} = f_4 \circ f_3 \circ f_2 \circ f_1(\mathbf{x})
% \end{equation}

% Along the same lines, we further emphasize the connection to iterative maps by simplifying our notation further by using a standard notational trick to turn the affine transformations normally used the neural network literature into more compact, but mathematically equivalent, linear transformations \cite{FIXME}. We perform this simplification by arranging the input data $x$ into a matrix $X$ where $X\in\mathbb{R}_{d \times n}$, which is commonly called a \emph{mini-batch}. We then have that $n$ is the number of input examples combined within a single matrix and $d$ is the dimension of $\mathbf{x}\in\mathbb{R}_{d \times 1}$.  Afterwards, we attach a single vector of $1$'s with dimension $1 \times n$ to the base of the input matrix $X$ so that the dimension $p$ of $X$ is the initial input dimension $d$ increased by $1$ as demonstrated in (\ref{eqn:xmatrix}) where $X\in\mathbb{R}_{p \times n}$.  By doing so, the weight matrix $A$ and bias $b$ may be concatenated into a single matrix $W$ where the final column contains the bias as demonstrated in \ref{eqn:wmatrix}.  The practice of attaching a vector of $1$'s to the base of the next layer's input matrix and concatenating the weights and biases into a single matrix occurs at each layer of the network.  The end result allows the overall notation to be simplified into the commonly used matrix notation shown in \ref{eqn:layerW}.

% \begin{equation}\label{eqn:xmatrix}
%     X=\begin{bmatrix}
%     x_{00} & \cdots & x_{0n}\\
%     \vdots & \ddots & \vdots\\
%     x_{d0} & \cdots & x_{dn}\\
%     1 & \cdots & 1
%     \end{bmatrix}
% \end{equation}

% \begin{equation}\label{eqn:wmatrix}
%     W_i=\begin{bmatrix}
%     A_{i_{00}} & \cdots & A_{i_{0d}} & b_0\\
%     \vdots & \ddots & \vdots & \vdots\\
%     A_{i_{j0}} & \cdots & A_{i_{jd}} & b_j
%     \end{bmatrix}
% \end{equation}

% \begin{equation}\label{eqn:layerW}
%     f_i(X)=\sigma(W_i \cdot X) 
% \end{equation}

% % The fundamental components of a feed-forward multilayer perceptron (MLP) \cite{MURTAGH1991183} form a starting point from which network structure may be specified through hyperparameter selection as shown in Fig. \ref{fig:mlpdiag} illustrating the case of a simple MLP with output dimension 1.   The field has expanded from this initial point to include many neural network architectures with unique design considerations.  Each evolution in neural network design offers complex structures and model characteristics allowing widespread adaptability to satisfy complex problems across many domains.  

% % \begin{figure}[htbp]
% %      \centering
% %      \includegraphics[width=0.5\textwidth]{Figures/mlpdiag.png}
% %      \caption{Two layer diagram of typical MLP architecture.}
% %      \label{fig:mlpdiag}
% % \end{figure}

% \subsection{MLPs as an iterative NN} \label{sec:MLPs_iterative}

% \begin{definition}
%     MLP as an iterative NN, i.e., equations \eqref{eqn:iteration1}  $\cdots$ \eqref{eqn:iteration3}
% \end{definition}

% The roots of iterative representations of neural networks are grounded in the tenets of dynamical systems theory. Dynamical systems theory encompasses a well-established field of mathematical study supported by an extensive body of research and theory \cite{nla.cat-vn1299669}. The area has proven well suited to complex systems including characteristics such as feedback and nonlinear behavior with famous examples including the Mandelbrot Set \cite{https://doi.org/10.1111/j.1749-6632.1980.tb29690.x} and fractal geometry \cite{MAN83}. Core features of dynamic systems include functional structures which iterate upon themselves \cite{SUGIE1991729, 1272974} to form feedback loops as denoted in \ref{eqn:nestedF} below.

% \begin{equation}\label{eqn:nestedF}
%     f \circ f \circ f \circ f(X)
% \end{equation}

% \noindent Note the similarity between \ref{eqn:nestedF} and \ref{eqn:nestedfx}.   The only difference is that one iterates a \emph{fixed} function in \ref{eqn:nestedF}, while one nest \emph{varying} functions in \ref{eqn:nestedfx}.

% In this section, MLPs are demonstrated to be another example of dynamical systems which may be expressed through iterative notation.  The visual similarities between the two functional structures from \ref{eqn:nestedf} and \ref{eqn:nestedF} are emblematic of an equivalence that may be made precise through some judicious notational choices.  Additionally, these models can be implemented using popular deep learning software environments in a manner that allows further study of iterative neural networks.  Within the context of this study, \textbf{Iterative Neural Network (INN)} \todo{What is the right thing to do here?  Are INNs really different thing from RNNs?  Are just forcing a name?} Architectures are defined as a broader class of networks in which the parameters are applied recursively against the input over multiple repetitions.  INNs are presented as a more generalized concept versus RNNs which typically feature dense parameter matrices, whereas the parameters of INNs may be arranged in a wide array of configurations including sparse configurations and self-contained layers.  The broader inspiration in demonstrating equivalence between INNs and MLPs would be the potential to leverage and benefit from the cross-application of dynamic systems principles and theory.  More directly, the restatement of traditional neural network architectures in an iterative format yields several immediate questions with clear implications for our understanding of the principles governing neural network structures. 

% As a first step, the problem may be approached by notationally restating the traditional neural network into a mathematically equivalent iterative function.  Beginning with a basic two-layer MLP feed-forward network and using the notational structure from \ref{eqn:nestedf}, the network can be depicted as the series of nested functions in \ref{eqn:nestedF}. Using the structure outlined in Section \ref{sec:method_mlp} applied to the two-layer case, we begin with the overall architecture of the two-layer MLP network as demonstrated in Fig. \ref{fig:layersmlp}, below.

% \begin{figure}[htbp]
%      \centering
%      \includegraphics[width=0.5\textwidth]{Figures/layersmlp.png}
%      \caption{Standard representation of a two-layer MLP.}
%      \label{fig:layersmlp}
% \end{figure}

% \begin{equation}\label{eqn:nestedmlp}
%     f_1\circ f_1(X)=\sigma(W_1\sigma(W_0 \cdot X))=Y
% \end{equation}

% Together, these component matrices will be used to compile a single iterative network function represented by the square matrix $f(X)$.  To begin, the component matrices $X$, $H$ and $Y$ are vertically concatenated together forming a single expanded input matrix $Z$ where $H$ and $Y$ are each initialized as zero matrices.  Using the stated dimensions from Section \ref{sec:method_mlp}, $X\in\mathbb{R}_{p \times n}$ with input dimension $p$ over $n$ examples.  Similarly, matrix $H$ shares the dimension of the hidden layer $h$ over $n$ examples and matrix $Y$ has output dimension $y$ across $n$ examples.  The resulting matrix $Z \in \mathbb{R}_{(p+h+y) \times n}$.  At this point a single square matrix $W \in \mathbb{R}_{(p+h+y) \times (p+h+y)}$ is initialized representing the iterative weight matrix, constructed in block-wise fashion using untrainable zero matrices with several exceptions.  The upper leftmost component matrix is initialized as an untrainable square identity matrix $I$ \todo{The mention of the identity here is jumping the gun I think, I mean this is needed for the RNN later, but not for the equivalence to the MLP which is discussed here} with each side matching the input dimension $p$.  Additionally, trainable weight matrices $W_0$ and $W_1$ are inserted as demonstrated in Fig. \ref{fig:iterativemlp}.  Finally, the matrix is wrapped in the relevant activation function as demonstrated in Fig. \ref{fig:iterativemlp} to form a combined representation of an iterative $f(X) = W \cdot X$.  The outcome is a single square parent matrix encompassing both weights matrices joined with regions composed of untrainable zero matrices wrapped in a pointwise nonlinearity function.  This specific case represents a single-encompassing iterative functional representation of the two-layer MLP example from Fig. \ref{fig:layersmlp}.  This square matrix $f(X)$ \todo{$f(X)$ is not a square matrix.  It contains a square matrix} is multiplied twice by the concatenated input matrix $Z$ reflecting a single iteration per layer of weights \todo{This description needs some work}.  The resulting output is mathematically identical to the initial feed-forward MLP that served as a starting point. Under this iterative representation, the region of $Z$ denoted as the $Y$ matrix continues to represent the output of the neural network just as the region denoted as $H$ continues to represent the output of a hidden layer.

% $$
% f(Z) = 
% \begin{blockarray}{ccccccc}
%  & & {\scriptstyle p} & {\scriptstyle h} & {\scriptstyle y} & & \\
% \begin{block}{cc[ccc][c]c}
%            & \rotatebox{90}{$\scriptstyle p$} & 0   & 0   & 0 &  \mathbf{x} &  \\
% \sigma_h ( & \rotatebox{90}{$\scriptstyle h$} & W_0 & 0   & 0 &  \mathbf{0} & )\\
% \sigma_y ( & \rotatebox{90}{$\scriptstyle y$} & 0   & W_1 & 0 &  \mathbf{0} & )\\
% \end{block}
% \end{blockarray}
% $$

% $$
% f(Z) = 
% \begin{blockarray}{ccccccc}
%  & & {\scriptstyle p} & {\scriptstyle h} & {\scriptstyle y} & & \\
% \begin{block}{cc[ccc][c]c}
%            & \rotatebox{90}{$\scriptstyle p$} & 0   & 0   & 0 &  \mathbf{0} &  \\
% \sigma_h ( & \rotatebox{90}{$\scriptstyle h$} & W_0 & 0   & 0 &  \sigma_h(W_0 \cdot \mathbf{x}) & )\\
% \sigma_y ( & \rotatebox{90}{$\scriptstyle y$} & 0   & W_1 & 0 &  \mathbf{0} & )\\
% \end{block}
% \end{blockarray}
% $$

% $$
% f(Z) = 
% \begin{blockarray}{ccccccc}
%  & & {\scriptstyle p} & {\scriptstyle h} & {\scriptstyle y} & & \\
% \begin{block}{cc[ccc][c]c}
%            & \rotatebox{90}{$\scriptstyle p$} & 0   & 0   & 0 &  \mathbf{0} &  \\
% \sigma_h ( & \rotatebox{90}{$\scriptstyle h$} & W_0 & 0   & 0 &  \mathbf{0} & )\\
% \sigma_y ( & \rotatebox{90}{$\scriptstyle y$} & 0   & W_1 & 0 &  \sigma_y(W_1 \cdot \sigma_h(W_0 \cdot \mathbf{x})) & )\\
% \end{block}
% \end{blockarray}
% $$



% \begin{figure}[htbp]
%      \centering
%      \includegraphics[width=0.5\textwidth]{Figures/iterative1.png}
%      \caption{Iterative Neural Network (INN) representation of a two-layer MLP.}
%      \label{fig:iterativemlp}
% \end{figure}

% $$
% f(Z) = 
% \begin{blockarray}{ccccccc}
%  & & {\scriptstyle p} & {\scriptstyle h} & {\scriptstyle y} & & \\
% \begin{block}{cc[ccc][c]c}
%            & \rotatebox{90}{$\scriptstyle p$} & I   & 0   & 0 &  \mathbf{x} &  \\
% \sigma_h ( & \rotatebox{90}{$\scriptstyle h$} & W_0 & 0   & 0 &  \mathbf{h} & )\\
% \sigma_y ( & \rotatebox{90}{$\scriptstyle y$} & 0   & W_1 & 0 &  \mathbf{y} & )\\
% \end{block}
% \end{blockarray}
% $$

% \todo{Can this be better done using LaTeX?}

% Following two iterative applications (once per layer) of this iterative neural network $f(Z)$, the resulting output is outlined in \ref{eqn:iterativemlp}.  It should be immediately clear that the resulting output is mathematically identical to the output denoted in \ref{eqn:nestedmlp} notationally bridging the perceived differences between Fig. \ref{fig:layersmlp} and Fig. \ref{fig:iterativemlp}.

% \begin{equation}\label{eqn:iterativemlp}
%     f(f(Z))=\sigma(W_1\sigma(W_0X))=Y
% \end{equation}



% \bigskip

% While the standard MLP neural network has proven to be a versatile and strong performer for many estimation and classification tasks, it suffers from the limitation of statelessness in that it retains no stored memory after each input example of the instances it has processed before.  For sequential data sets which take place either as part of a greater whole or which hold some relationship with the surrounding members in a given sequence, memory is clearly a desirable or even necessary trait.  For these cases there exist many architectures for analyzing data in series, among which are the Recurrent Neural Network (RNN) and the Long Short-Term Memory Network (LSTM) which are discussed next.

% \subsection{Sequential2D} \label{sec:sequential_2D}

% In this paper, we leverage a novel deep-learning container Sequential2D. Similar to Pytorch's Sequential which organizes the building blocks of complex neural networks and serves as architectural aid for many complex neural networks such as GPT-2.  We propose Sequential2D as an enhanced orchestrator which provides insights into not only the width and depth of the network but also the skip connections.  A precise mathematical definition of Sequential2D can be found in (\ref{eq:long-eq}).

% In (\ref{eq:long-eq}) each $f_{ij}$ is some arbitrary non-linear function and the $\circ$ operator is function composition (or in this case function application) operator.  In many ways, (\ref{eq:long-eq}) is a straight forward generalization of a block defined matrix.  In particular, if every function $f_{ij}$ happened to be linear (i.e., a matrix) and the function composition operator $\circ$ were replaced with the dot-product, then (\ref{eq:long-eq}) would be precisely a block defined matrix.  
% \emph{So, the \textbf{2D} in Sequential2D refers to the 2D matrix of functions, as opposed to the 1D array of functions in a Pytorch or Keras Sequential container.}  
% Specifically, Sequential2D is a PyTorch module that allows you to define a neural network by specifying a sequence of layers. The layers are defined as a list of PyTorch modules, which can be any type of layer or operation supported by PyTorch \cite{pytorch2017automatic}.
% Sequential2D can be used with a variety of neural network models, including MLPs, RNNs, LSTMs, transformers, and convolutional neural networks.

% Of course, we are not the first to propose thinking about neural networks in terms of a block matrix structure.  For example, the work by \cite{narang2017blocksparse} provides a promising approach for reducing the size and computational complexity of RNNs without sacrificing accuracy. Their block-sparse RNNs could be used to make RNNs more accessible to a wider range of applications, and could also be used to improve the performance of RNNs on existing applications. Further, in \cite{narang2017blocksparse} the authors observe that block sparsity is a more structured form of sparsity than unstructured sparsity\footnote{Structured sparsity refers to a specific pattern of zeros in a sparse matrix, while unstructured sparsity lacks any regularity in the distribution of zeros. Block sparsity is a form of structured sparsity where zeros appear in contiguous blocks.}, and can lead to better performance on hardware architectures that support block-sparse matrix multiplication.

% There are two points that we wish to emphasize:

% \begin{itemize}
%     \item As can be seen in (\ref{eq:long-eq}) there is additional information propagation in a Sequential2D that is not possible in a standard Sequential container.  For example, the output $Y$ depends on $f_{m,0}(X) + f_{m,1}(H) + \hdots + f_{m,n}(Y)$ and not just $f_{m,n-1}(H_k)$ and it is precisely such information propagation that is required for SC.
%     \item As we will demonstrate in the next section, a Sequential2D neural network
%     can be thought of as an RNN, in that a fixed Sequential2D is iterated across a given data set.      
%     % and understanding the iterative structure of a Sequential2D is important for understanding the applications of Sequential2D.  In particular, in the next section we will demonstrate a close connection between Sequential2D, RNNs, and SC.
% \end{itemize}

% % Mathematically, Sequential2d is a rectangular block matrix function within which each entry is a matrix function. Perhaps this idea is best explained mathematically, here in (\ref{tab:long-eq}). Note, here dot products are replaced by function compositions which is exactly what we see as a key operation in neural networks. These compositions are often expressed using $\circ$ notation. 

% % A matrix is a rectangular array of numbers treated as a single object. A block matrix is a matrix whose elements are themselves matrices, which are called submatrices. By allowing a matrix to be viewed at different levels of abstraction, the block matrix viewpoint enables elegant proofs of results and facilitates the development and understanding of numerical algorithms. Block matrices can represent many complex linear transformations and has many applications in linear algebra.  


% \subsection{ToyGPT expressed using Sequential2D} \label{sec:toygpt}
% To make the use of a Sequential2D container concrete, we provide a simple example using the ToyGPT model from (\ref{eqn:gptmini}), and demonstrate now a
% Sequential2D can be interpreted as an RNN.

% % in we use three matrices, $X$, $H$, and $Y$, to create a single network function (Sequential2D) represented by the square matrix $f(Z)$. To do this, we vertically concatenate $X, H, Y$ together to form an expanded input matrix, $Z$. $X$ has dimension $p × n$ these are similar to the features of any dataset. Then, $H$ has dimension $h × n$ is the hidden representation and can be configured by the user, we keep them as $0$ vector throughout the paper. $Y$ has dimension $y × n$, we reserve this last position of predicted outputs. The function matrix  $f(Z)$ has dimension $(p+h+y) \times n$. Following is an $3x3$ example of Sequential2D but like any other matrix function this can be of any dimension $mxn$. In this paper, we will show more examples of varying dimensions and recast GPT2 using this framework. 

% In particular, ToyGPT is recast as shown in Equation-\ref{eqn:gptmini} using Sequential2D. Here we keep all the decoder blocks on the subdiagonal of the matrix and $X$ we defined earlier in this section.  The subdiagonal of a square matrix is the set of elements directly under the elements comprising the diagonal.  
% \emph{We then use Sequential2D as an iterative map and show three iterations yields the exact same mathematical output as ToyGPT Equation-\ref{eqn:gptmini}.}  More specifically, consider the following Sequential2D container.

% \begin{equation}
% \begin{aligned}
% \begin{bmatrix}
%     0 &
%     0 &
%     0 &
%     0 \\
%     f_{\theta_1} &
%     0 &
%     0 &
%     0 \\
%     0 &
%     f_{\theta_2} &
%     0 &
%     0 \\
%     0 &
%     0 &
%     L &
%     0 \\
% \end{bmatrix}
%     \circ
% \begin{bmatrix}
%     X \\
%     0 \\
%     0 \\
%     0
% \end{bmatrix} 
% & = 
% \begin{bmatrix}
% 0 \\
% f_{\theta_1}(X) \\
% 0 \\
% 0 \\
% \end{bmatrix}.
% \end{aligned}
% \label{eqn:iteration1}
% \end{equation}

% \noindent Note that applying the Sequential2D container to the input vector $X$, as in (\ref{eqn:iteration1}) leads to applying the first GPT2 layer to $X$ and placing the result of that computation into the \emph{second} entry of the output vector.  We can then apply the \emph{same} Sequential2D container to the output of the first application of the Sequential2D container. 

% \begin{equation}
% \begin{aligned}
% \begin{bmatrix}
%     0 &
%     0 &
%     0 &
%     0 \\
%     f_{\theta_1} &
%     0 &
%     0 &
%     0 \\
%     0 &
%     f_{\theta_2} &
%     0 &
%     0 \\
%     0 &
%     0 &
%     L &
%     0 \\
% \end{bmatrix}
%     \circ
% \begin{bmatrix}
%     0 \\
%     f_{\theta_1}(X) \\
%     0 \\
%     0
% \end{bmatrix} 
% & = 
% \begin{bmatrix}
% 0 \\
% 0 \\
% f_{\theta_2}(f_{\theta_1}(X)) \\
% 0 \\
% \end{bmatrix}. 
% \end{aligned}
% \label{eqn:iteration2}
% \end{equation}

% \noindent After applying the \emph{same} Sequential2D container in (\ref{eqn:iteration1}) we now have in the \emph{third} entry of the output vector containing the application of the first and second GPT-2 layers.

% \begin{equation}
% \begin{aligned}
% \begin{bmatrix}
%     0 &
%     0 &
%     0 &
%     0 \\
%     f_{\theta_1} &
%     0 &
%     0 &
%     0 \\
%     0 &
%     f_{\theta_2} &
%     0 &
%     0 \\
%     0 &
%     0 &
%     L &
%     0 \\
% \end{bmatrix}
%     \circ
% \begin{bmatrix}
%     0 \\
%     0 \\
%     f_{\theta_2}(f_{\theta_1}(X)) \\
%     0 \\
% \end{bmatrix} 
% & = 
% \begin{bmatrix}
%     0 \\
%     0 \\
%     0 \\
%     L(f_{\theta_2}(f_{\theta_1}(X))) \\
% \end{bmatrix} 
% \end{aligned}.
% \label{eqn:iteration3}
% \end{equation}

% \noindent After applying the \emph{same} Sequential2D container in (\ref{eqn:iteration1}) a third time we now have in the \emph{last} entry of the output vector containing \emph{exactly the same output as (\ref{eqn:gptmini})}.

% In the standard PyTorch training method, the forward pass involves propagating the input data through the layers of the network in a single step, followed by loss calculation. In contrast, with Sequential2D we train neural networks in an iterative fashion. We propagate the input data through the network, block-by-block, using blocks on the first sub-diagonal, with the output of each block being fed as input to the next. \emph{These iterations or the block-by-block information propagation constitute the second dimension (2D) in Sequential2D}. For example, $G_{0}(X)$ is the input to $f_{\theta_2}(X)$ with this process repeated for each layer in the network.  For networks with more than one layer this results in multiple iterations before loss calculation and backpropagation are performed using Pytorch's autograd \cite{pytorch2017automatic}.  

% The connection to block defined RNNs can be seen in equations (\ref{eqn:iteration1}), (\ref{eqn:iteration2}), and (\ref{eqn:iteration3}).  In fact, a Sequential2D is precisely a RNN, in which a typical Sequential container happens to be embedded onto to the first sub-diagonal of the Sequential2D container.  It follows to ask, what about the other blocks in the Sequential2D container?  As the next Section demonstrates, that is precisely where SC naturally arise.

% \subsection{Sparse Skip Connection} \label{sec:sparse_skip_connection}

% While deriving this sparse block representation of ToyGPT, it may be observed that there are many empty kernel or zero matrix functions. In the following sections, this research shows both mathematically and empirically the effectiveness of these zero matrix functions when permitted to train. 

% Equation-\ref{eqn:skipiteration3} demonstrates how a skip function may be derived by altering two zero blocks. By first specifying block (0,0) as an Identity block $I$ and block (3, 0) as trainable weights $S$ before performing three iterations with initial input $[X,0,0,0]$, the the resulting output is the skip connection between input $X$ and output of ToyGPT. We notice the dimension of block $S$ is huge, i.e. around 150M $(768 \times 16) \times (768 \times 16)$, we allow only a fraction of the weights to train. There are many ways sparsity can be introduced in a network \cite{sparse_survey}. In parallel, we develop a masked linear layer in PyTorch allowing the network to prevent weights from training during backpropagation. 
% \begin{equation}\label{masked_linear}
%     S = U \odot \Omega + W    
% \end{equation}
% The linear mask is shown in (\ref{masked_linear}), which takes the Hadamard product of $U$ containing the gradients and $\Omega$ containing the integer boolean mask before adding $W$ which contains the initial weights.  Note, if $\Omega$ is a matrix of ones then one can show above equation is the same as a Linear layer \cite{pytorch2017automatic, chollet2015keras}. After applying this Sparse skip connection, we choose randomly choose 800k parameters to train out of 150M.

  

% \begin{equation}
% \begin{aligned}
% \begin{bmatrix}
%     I &
%     0 &
%     0 &
%     0 \\
%     f_{\theta_1} &
%     0 &
%     0 &
%     0 \\
%     0 &
%     f_{\theta_2} &
%     0 &
%     0 \\
%     S &
%     0 &
%     L &
%     0 \\
% \end{bmatrix}
%     \circ
%     \hdots
%     \circ
% \begin{bmatrix}
%     I &
%     0 &
%     0 &
%     0 \\
%     f_{\theta_1} &
%     0 &
%     0 &
%     0 \\
%     0 &
%     f_{\theta_2} &
%     0 &
%     0 \\
%     S &
%     0 &
%     L &
%     0 \\
% \end{bmatrix}
%     \circ
% \begin{bmatrix}
%     X \\
%     0 \\
%     0 \\
%     0 \\
% \end{bmatrix} 
% % \begin{bmatrix}
% %     X \\
% %     f_{\theta_1}(X) \\
% %     f_{\theta_2}(f_{\theta_1}(X)) \\
% %     S(X) \\
% % \end{bmatrix} 
% & = 
% \begin{bmatrix}
%     X \\
%     f_{\theta_1}(X) \\
%     f_{\theta_2}(f_{\theta_1}(X)) \\
%     S(X) +\\ L(f_{\theta_2}(f_{\theta_1}(X))) \\
% \end{bmatrix} 
% \end{aligned}
% \label{eqn:skipiteration3}
% \end{equation}


% \subsection{Generalizations of the iterative MLP} \label{sec:generalization_MLP}
% The INN representation of the neural network makes explicit the untrainable zero matrices surrounding the weight matrices which are implied in the traditional feed-forward MLP and other typical feed-forward networks.  Together, the regions of the weight matrix are horizontally aligned with the trainable weights as depicted in Fig. \ref{fig:iterativeweightspace} form the \textbf{weight space}.  Each parameter within the weight space shares the common characteristic of being subject to the pointwise application of the nonlinearity function $\sigma$, with the potential to be parameterized and function as a trainable weight across broader applications of the iterative function in alternative configurations.

% \begin{figure}[htbp]
%      \centering
%      \includegraphics[width=0.5\textwidth]{Figures/iterative02.png}
%      \caption{INN representation of a two-layer MLP with the structure of the weight space expanded to include all regions horizontally adjacent to the weight matrices $W_0$ and $W_1$.}
%      \label{fig:iterativeweightspace}
% \end{figure}

% $$
% f(Z) = 
% \begin{blockarray}{ccccccc}
%  & & {\scriptstyle p} & {\scriptstyle h} & {\scriptstyle y} & & \\
% \begin{block}{cc[ccc][c]c}
%            & \rotatebox{90}{$\scriptstyle p$} & I   & 0   & 0   &  \mathbf{x} &  \\
% \sigma_h ( & \rotatebox{90}{$\scriptstyle h$} & W_0 & W_2 & W_3 &  \mathbf{h} & )\\
% \sigma_y ( & \rotatebox{90}{$\scriptstyle y$} & W_4 & W_1 & W_5 &  \mathbf{y} & )\\
% \end{block}
% \end{blockarray}
% $$

% we call the below the \emph{weight space}

% $$
% \begin{blockarray}{ccc}
% \begin{block}{[ccc]}
% W_0 & W_2 & W_3 \\
% W_4 & W_1 & W_5 \\
% \end{block}
% \end{blockarray}
% $$



% Having established the ability for the iterative matrix to replicate a traditional feed-forward MLP and achieve mathematical equivalence an additional consideration lies with implementation.  The identity matrix $I$ and zero matrices located above the weight space within the iterative matrix in Fig. \ref{fig:iterativeweightspace} serve the purpose of returning the input component matrix $X$ to the larger matrix $Z$ made possible by the absence of pointwise nonlinearity $\sigma$.  An alternate but equivalent approach to implementation removes portions of the iterative matrix lying above the weight space as depicted in Fig. \ref{fig:iterativeweightspace2}.  Instead, the function of the deleted identity matrix is performed prior to each iteration by inserting a copy of the initial input component matrix $X$ into the matrix $Z$.  Approaching the network in this manner recasts the input $X$ as a sequence of identical steps, with each step comprised of duplicate copies of $X$.  Rather than specifying iterations independently of the input, the network now iterates over each step $X_t$ within the sequence $X$ with one occurrence per layer while the output remains the same.  Sequential notation is adopted across the model to differentiate output at each time step $t$ resulting in $Z_{t}$ composed of $X_t$, $H_t$ and $Y_t$.

% \begin{figure}[htbp]
%      \centering
%      \includegraphics[width=0.5\textwidth]{Figures/weightspace01.png}
%      \caption{Alternate implementation of iterative network replicating a two-layer MLP truncated to include only the weight space with the input component matrix $X$ inserted into the larger input matrix $Z$ prior to each iteration.}
%      \label{fig:iterativeweightspace2}
% \end{figure}

% $$
% f(Z) = 
% \begin{blockarray}{ccccccc}
% \begin{block}{cc[ccc][c]c}
%            & & & & &  \mathbf{x} &  \\
% \sigma_h ( & \rotatebox{90}{$\scriptstyle h$} & W_0 & W_2 & W_3 &  \mathbf{h} & )\\
% \sigma_y ( & \rotatebox{90}{$\scriptstyle y$} & W_4 & W_1 & W_5 &  \mathbf{y} & )\\
% \end{block}
% \end{blockarray}
% $$

% Within the weight space, the design choice to define the matrices surrounding each MLP layer as untrainable zero matrices is an implied decision and form an unnecessary constraint.  This recognition gives rise to questioning whether other and perhaps better alternatives exist and what principles may govern the optimal definition of architectures within those regions.  As one example, initializing some combination of the matrices along the diagonal of the iterative matrix with untrainable identity matrices allows the function $f(X)$ to retain persistent memory of the data contained in each region of $Z$ for each iteration of $f(Z)$.  The immediate impact of this change would appear to be minor within the scope of the overall network but creates new capabilities and allows the network to perform when iterations exceed the number of layers.  By retaining memory at each step, data from each prior iteration continues to factor into model training and output.  However, this change is simply one of many possibilities with the matrices capable of being initialized in any number of combinations and configurations.  Importantly, the choice of matrix trainability within the weight space represents yet another hyperparameter to be optimized and studied.  This same line of reasoning can be extended to both the zero matrices lying above the diagonal drawing information backward through the model and the zero matrices below the diagonal which can serve as skip connections.  These characteristics underscore the inherent flexibility of the INN architecture, presented here as a more generalized version of the MLP.  Taking the idea a step further, the parent matrix $f(X)$ may be arbitrarily subdivided with granularity as fine as individual parameters allowing detailed specification of network structure.  This capability enables the INN architecture to replicate other model types while also exploring the impact of parameterization on model performance.


==> sections/old/ConvergentNeuralNetworks_old.tex <==
% Put S above the diagonal
% Show that the RNN now converges as a function of S

\section{Exploring full generality of iterated maps}
This opens an entire range of new possibilities when considering a block iterative function of the form

% Full matrix
\begin{equation} \label{eq:GEN_all}
    \begin{bmatrix}
        \Wy{W_{1,1}} & \Wr{W_{1,2}}  & \Wr{W_{1,3}}  & \Wr{W_{1,4}}  & \Wr{W_{1,5}} \\
        \Wg{W_{2,1}} & \Wy{W_{2,2}}  & \Wr{W_{2,3}}  & \Wr{W_{2,4}}  & \Wr{W_{2,5}} \\
        \Wb{W_{3,1}} & \Wg{W_{3,2}}  & \Wy{W_{3,3}}  & \Wr{W_{3,4}}  & \Wr{W_{3,5}} \\
        \Wb{W_{4,1}} & \Wb{W_{4,2}}  & \Wg{W_{4,3}}  & \Wy{W_{4,4}}  & \Wr{W_{4,5}} \\
        \Wb{W_{5,1}} & \Wb{W_{5,2}}  & \Wb{W_{5,3}}  & \Wg{W_{5,4}}  & \Wy{W_{5,5}} \\
    \end{bmatrix}
\end{equation}

In this notation, 

\begin{itemize}
\item $\Wg{W_{i+1,i}}$ corresponds to a standard MPL or, more generally, an NN that can be implemented as a Pytorch or Keras Sequential container.
\item $\Wb{W_{i+k,i}}, \; k>1$ corresponds to skip connections and finite impulse response (FIR) filters.
\item We began the exploration of $\Wy{W_{i,i}}$ with the introduction of the $I$ in \eqref{FIXME} corresponds infinite impulse response filters.
\item What do $\Wr{W_{i,j}}, \; j>i$ correspond to?  They are actually \emph{feedback} connections which also lead to infinite impulse response filters and classic RNNs.
\end{itemize}

\subsection{On the diagonal}

\begin{equation}
M_d = 
  \left[
      \begin{matrix}
  \Wy{I} & 0 & 0 & 0\\
  \myfone & \Wy{S} & 0 & 0\\
  0 & \myftwo & 0 & 0\\
  0 & 0 & \myfthr & 0
      \end{matrix}
    \right]
  \end{equation}
  
  \begin{equation}
    \circ_{i=1}^3 M_{d}  
    \left(
      \begin{bmatrix}
          \mv{x} \\
          0 \\
          0 \\
          0 \\
      \end{bmatrix}
      \right) = 
    \left[
      \begin{matrix}
  \mv{x} \\
  \left(\Wy{S} \circ \myfone \circ \mv{x} +  \Wy{S} \circ \Wy{S} \circ \myfone \circ \mv{x} +  \myfone \circ \mv{x} \right) \\
  \left(\myftwo \circ \Wy{S} \circ \myfone \circ \mv{x} +  \myftwo \circ \myfone \circ \mv{x} \right) \\
  \myfthr \circ \myftwo \circ \myfone \circ \mv{x} 
      \end{matrix}
    \right]
  \end{equation}
  
  \begin{equation}
    \circ_{i=1}^4 M_{d}  
    \left(
      \begin{bmatrix}
          \mv{x} \\
          0 \\
          0 \\
          0 \\
      \end{bmatrix}
      \right) = 
    \left[
      \begin{matrix}
  \mv{x} \\
  \left(\Wy{S} \circ \myfone \circ \mv{x} +  \Wy{S} \circ \Wy{S} \circ \myfone \circ \mv{x} +  \Wy{S} \circ \Wy{S} \circ \Wy{S} \circ \myfone \circ \mv{x} +  \myfone \circ \mv{x} \right) \\
  \left(\myftwo \circ \Wy{S} \circ \myfone \circ \mv{x} +  \myftwo \circ \Wy{S} \circ \Wy{S} \circ \myfone \circ \mv{x} +  \myftwo \circ \myfone \circ \mv{x} \right) \\
  \left(\myfthr \circ \myftwo \circ \Wy{S} \circ \myfone \circ \mv{x} +  \myfthr \circ \myftwo \circ \myfone \circ \mv{x} \right) 
      \end{matrix}
    \right]
  \end{equation}

  In general, after the $k$-th iteration, if $S$ and $f_{\theta_i}$ are linear, with $k \ge 3$ we have

  \begin{equation}
    \circ_{i=1}^k M_{d}  
    \left(
      \begin{bmatrix}
          \mv{x} \\
          0 \\
          0 \\
          0 \\
      \end{bmatrix}
      \right) = 
    \left[
      \begin{matrix}
  \mv{x} \\
  ( \circ_{i=0}^{k-1} \Wy{S} ) \circ \myfone \circ \mv{x} \\
  \myftwo \circ ( \circ_{i=0}^{k-2} \Wy{S} ) \circ \myfone \circ \mv{x} \\
  \myfthr \circ \myftwo \circ ( \circ_{i=0}^{k-3} \Wy{S} ) \circ \myfone \circ \mv{x} 
      \end{matrix}
    \right]
  \end{equation}

So, in the linear case, the convergence of the above is determined by the convergence of the infinite product of $S$ alone!  I.e., if we choose $S$ \emph{and} the $f{\theta_i}$ to be a linear function  where the power-series is well understood.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Above the diagonal}

\begin{equation}
  M_{ad} = 
    \left[
      \begin{matrix}
  \myI & 0 & 0 & 0\\
  \myfone & 0 & \myS & 0\\
  0 & \myftwo & 0 & 0\\
  0 & 0 & \myfthr & 0
      \end{matrix}
    \right]
  \end{equation}
  
  \begin{equation}
    \circ_{i=1}^{3}M_{ad}  
    \left(
      \begin{bmatrix}
          \mv{x} \\
          0 \\
          0 \\
          0 \\
      \end{bmatrix}
      \right) = 
      \left[
      \begin{matrix}
  \mv{x} \\
  \left(\myS \circ \myftwo \circ \myfone \circ \mv{x} +  \myfone \circ \mv{x} \right) \\
  \myftwo \circ \myfone \circ \mv{x} \\
  \myfthr \circ \myftwo \circ \myfone \circ \mv{x} 
      \end{matrix}
    \right]
  \end{equation}
  
  \begin{equation}
    \circ_{i=1}^{4}M_{ad}  
    \left(
      \begin{bmatrix}
          \mv{x} \\
          0 \\
          0 \\
          0 \\
      \end{bmatrix}
      \right) = 
    \left[
      \begin{matrix}
  \mv{x} \\
  \left(\myS \circ \myftwo \circ \myfone \circ \mv{x} +  \myfone \circ \mv{x} \right) \\
  \left(\myftwo \circ \myS \circ \myftwo \circ \myfone \circ \mv{x} +  \myftwo \circ \myfone \circ \mv{x} \right) \\
  \myfthr \circ \myftwo \circ \myfone \circ \mv{x} 
      \end{matrix}
    \right]
  \end{equation}
  
  \begin{equation}
    \circ_{i=1}^{5}M_{ad}  
    \left(
      \begin{bmatrix}
          \mv{x} \\
          0 \\
          0 \\
          0 \\
      \end{bmatrix}
      \right) = 
    \left[
      \begin{matrix}
  \mv{x} \\
  \left(\myS \circ \myftwo \circ \myS \circ \myftwo \circ \myfone \circ \mv{x} +  \myS \circ \myftwo \circ \myfone \circ \mv{x} +  \myfone \circ \mv{x} \right) \\
  \left(\myftwo \circ \myS \circ \myftwo \circ \myfone \circ \mv{x} +  \myftwo \circ \myfone \circ \mv{x} \right) \\
  \left(\myfthr \circ \myftwo \circ \myS \circ \myftwo \circ \myfone \circ \mv{x} +  \myfthr \circ \myftwo \circ \myfone \circ \mv{x} \right) 
      \end{matrix}
    \right]
  \end{equation}
  
  In general, after the $k$-th iteration, if $S$ and $f_{\theta_i}$ are linear, with $k$ odd and $k \ge 3$ we have

  \begin{equation}
    \circ_{i=1}^{k} M_{ad}  
    \left(
      \begin{bmatrix}
          \mv{x} \\
          0 \\
          0 \\
          0 \\
      \end{bmatrix}
      \right) = 
    \left[
      \begin{matrix}
  \mv{x} \\
  ( \circ_{i=0}^{\frac{k-1}{2}} (\myS \circ \myftwo) ) \circ \myfone \circ \mv{x} \\
  \myftwo \circ ( \circ_{i=0}^{\frac{k-3}{2}} (\myS \circ \myftwo) ) \circ \myfone \circ \mv{x} \\
  \myfthr \circ \myftwo \circ ( \circ_{i=0}^{\frac{k-3}{2}} (\myS \circ \myftwo) ) \circ \myfone \circ \mv{x} 
      \end{matrix}
    \right]
  \end{equation}

After the $k$-th iteration, if $S$ and $f_{\theta_i}$ are linear, with $k$ even and $k \ge 4$ we have

  \begin{equation}
    \circ_{i=1}^{k} M_{ad}  
    \left(
      \begin{bmatrix}
          \mv{x} \\
          0 \\
          0 \\
          0 \\
      \end{bmatrix}
      \right) = 
    \left[
      \begin{matrix}
  \mv{x} \\
  ( \circ_{i=0}^{\frac{k-3}{2}} (\myS \circ \myftwo) ) \circ \myfone \circ \mv{x} \\
  \myftwo \circ ( \circ_{i=0}^{\frac{k-3}{2}} (\myS \circ \myftwo) ) \circ \myfone \circ \mv{x} \\
  \myfthr \circ \myftwo \circ ( \circ_{i=0}^{\frac{k-4}{2}} (\myS \circ \myftwo) ) \circ \myfone \circ \mv{x} 
      \end{matrix}
    \right]
  \end{equation}

So, in the liner case, the convergence of the above is determined by the convergence of the infinite product of $S \circ \myftwo$ alone!  Note, here $\myftwo$, and the $f_{\theta_i}$, are generally non-linear functions and the power-series is not available in closed form.  However, perhaps special cases of $f_{\theta_i}$ can be considered.

\subsection{RNN picture}

Recall \eqref{eq:RNN_DS_RHS}
% Full matrix
\begin{equation}
    \begin{bmatrix}
        0 & 0  & 0  & 0  & 0 \\
        \Wg{W_{2,1}} & \Wy{W_{2,2}}  & \Wr{W_{2,3}}  & \Wr{W_{2,4}}  & \Wr{W_{2,5}} \\
        \Wb{W_{3,1}} & \Wg{W_{3,2}}  & \Wy{W_{3,3}}  & \Wr{W_{3,4}}  & \Wr{W_{3,5}} \\
        \Wb{W_{4,1}} & \Wb{W_{4,2}}  & \Wg{W_{4,3}}  & \Wy{W_{4,4}}  & \Wr{W_{4,5}} \\
        \Wb{W_{5,1}} & \Wb{W_{5,2}}  & \Wb{W_{5,3}}  & \Wg{W_{5,4}}  & \Wy{W_{5,5}} \\
    \end{bmatrix}
    =
    \begin{bmatrix}
        0 & 0 \\
        W_1 & W_2 \\
    \end{bmatrix}
\end{equation}


% % Above the diagonal
% For example
% \begin{equation}
% \begin{aligned}
%     &\begin{bmatrix}
%         \Wy{I}   & \Wr{H_0}  & 0      & 0 \\
%         \Wg{f_{\theta_1}} & 0         & 0      & 0 \\
%         0         & \Wg{f_{\theta_2}} & 0      & 0 \\
%         \Wb{S}   & 0         & \Wg{f_{\theta_3}} & 0 \\
%     \end{bmatrix}
%     \circ 
%    \begin{bmatrix}
%         \Wy{I}   & \Wr{H_0}  & 0      & 0 \\
%         \Wg{f_{\theta_1}} & 0         & 0      & 0 \\
%         0         & \Wg{f_{\theta_2}} & 0      & 0 \\
%         \Wb{S}   & 0         & \Wg{f_{\theta_3}} & 0 \\
%     \end{bmatrix}
%     \circ
%     \begin{bmatrix}
%         \Wy{I}   & \Wr{H_0}  & 0      & 0 \\
%         \Wg{f_{\theta_1}} & 0         & 0      & 0 \\
%         0         & \Wg{f_{\theta_2}} & 0      & 0 \\
%         \Wb{S}   & 0         & \Wg{f_{\theta_3}} & 0 \\
%     \end{bmatrix}
%         \circ
%     \begin{bmatrix}
%         X \\
%         0 \\
%         0 \\
%         0 \\
%     \end{bmatrix} 
%     = \\ \\
%     & \hspace{1cm}
%     \begin{bmatrix}
%         X + 2 H_0(f_{\theta_1}(X)) \\
%         f_{\theta_1}(X) + f_{\theta_1}(H_0(f_{\theta_1}(X))) \\
%         f_{\theta_2}(f_{\theta_1}(X)) \\
%         S(X) +S(H_0(f_{\theta_1}(X))) + f_{\theta_3}(f_{\theta_2}(f_{\theta_1}(X))) \\
%     \end{bmatrix} 
%     \label{eqn:skipiterationcolor}
% \end{aligned}
% \end{equation}

% This is not a fixed point. Discuss sparsity




==> sections/old/Generalizations.tex <==

\subsection{Diagonal blocks} \label{sec:generalizations-diagonal}

Let
\begin{equation}\label{eq:generalizations-diagonal}
M_{d4} = 
  \left[
      \begin{matrix}
  \Wy{I} & 0 & 0 & 0\\
  \myfone & \Wy{S} & 0 & 0\\
  0 & \myftwo & 0 & 0\\
  0 & 0 & \myfthr & 0
      \end{matrix}
    \right]
  \end{equation}

Note that after three iterations
  \begin{equation} \label{eq:generalizations-diagonal-M3-iteration3}
    \circ_{i=1}^3 M_{d}  
    \left(
      \begin{bmatrix}
          \mv{h}_0 \\
          0 \\
          0 \\
          0 \\
      \end{bmatrix}
      \right) = 
    \left[
      \begin{matrix}
  \mv{h}_0 \\
  \left(\Wy{S} \circ \myfone \circ \mv{h}_0 +  \Wy{S} \circ \Wy{S} \circ \myfone \circ \mv{h}_0 +  \myfone \circ \mv{h}_0 \right) \\
  \left(\myftwo \circ \Wy{S} \circ \myfone \circ \mv{h}_0 +  \myftwo \circ \myfone \circ \mv{h}_0 \right) \\
  \myfthr \circ \myftwo \circ \myfone \circ \mv{h}_0 
      \end{matrix}
    \right]
  \end{equation}
After four iterations
  \begin{equation} \label{eq:generalizations-diagonal-M3-iteration3}
    \circ_{i=1}^4 M_{d}  
    \left(
      \begin{bmatrix}
         \mv{h}_0 \\
          0 \\
          0 \\
          0 \\
      \end{bmatrix}
      \right) = 
    \left[
      \begin{matrix}
  \mv{h}_0 \\
  \left(\Wy{S} \circ \myfone \circ \mv{h}_0 +  \Wy{S} \circ \Wy{S} \circ \myfone \circ \mv{h}_0 +  \Wy{S} \circ \Wy{S} \circ \Wy{S} \circ \myfone \circ \mv{h}_0 +  \myfone \circ \mv{h}_0 \right) \\
  \left(\myftwo \circ \Wy{S} \circ \myfone \circ \mv{h}_0 +  \myftwo \circ \Wy{S} \circ \Wy{S} \circ \myfone \circ \mv{h}_0 +  \myftwo \circ \myfone \circ \mv{h}_0 \right) \\
  \left(\myfthr \circ \myftwo \circ \Wy{S} \circ \myfone \circ \mv{h}_0 +  \myfthr \circ \myftwo \circ \myfone \circ \mv{h}_0 \right) 
      \end{matrix}
    \right]
  \end{equation}
In general, after the $k$-th iteration, if $S$ and $f_{\theta_i}$ are linear, with $k \ge 3$ we have
  \begin{equation} \label{eq:generalizations-diagonal-M3-iterationk}
    \circ_{i=1}^k M_{d}  
    \left(
      \begin{bmatrix}
          \mv{h}_0 \\
          0 \\
          0 \\
          0 \\
      \end{bmatrix}
      \right) = 
    \left[
      \begin{matrix}
  \mv{h}_0 \\
  ( \circ_{i=0}^{k-1} \Wy{S} ) \circ \myfone \circ \mv{h}_0 \\
  \myftwo \circ ( \circ_{i=0}^{k-2} \Wy{S} ) \circ \myfone \circ \mv{h}_0 \\
  \myfthr \circ \myftwo \circ ( \circ_{i=0}^{k-3} \Wy{S} ) \circ \myfone \circ \mv{h}_0 
      \end{matrix}
    \right]
  \end{equation}

So, in the linear case, the convergence of the above as $k \longmapsto \infty$ is determined by the convergence of the infinite product of $S$ alone, i.e., if we choose $S$ \emph{and} the $f_{\theta_j}$ to be a linear function  where the power-series is well understood.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Super-diagonal blocks} \label{sec:generalizations-superdiagonal}

Now consider
\begin{equation} \label{eq:generalizations-superdiagonal-M4}
  M_{ad} = 
    \left[
      \begin{matrix}
  \myI & 0 & 0 & 0\\
  \myfone & 0 & \myS & 0\\
  0 & \myftwo & 0 & 0\\
  0 & 0 & \myfthr & 0
      \end{matrix}
    \right]
  \end{equation}
  
  \begin{equation} \label{eq:generalizations-superdiagonal-M4-iteration3}
    \circ_{i=1}^{3}M_{ad}  
    \left(
      \begin{bmatrix}
          \mv{h}_0 \\
          0 \\
          0 \\
          0 \\
      \end{bmatrix}
      \right) = 
      \left[
      \begin{matrix}
  \mv{h}_0 \\
  \left(\myS \circ \myftwo \circ \myfone \circ \mv{h}_0 +  \myfone \circ \mv{h}_0 \right) \\
  \myftwo \circ \myfone \circ \mv{h}_0 \\
  \myfthr \circ \myftwo \circ \myfone \circ \mv{h}_0 
      \end{matrix}
    \right]
  \end{equation}
  
  \begin{equation} \label{eq:generalizations-superdiagonal-M4-iteration4}
    \circ_{i=1}^{4}M_{ad}  
    \left(
      \begin{bmatrix}
          \mv{h}_0 \\
          0 \\
          0 \\
          0 \\
      \end{bmatrix}
      \right) = 
    \left[
      \begin{matrix}
  \mv{h}_0 \\
  \left(\myS \circ \myftwo \circ \myfone \circ \mv{h}_0 +  \myfone \circ \mv{h}_0 \right) \\
  \left(\myftwo \circ \myS \circ \myftwo \circ \myfone \circ \mv{h}_0 +  \myftwo \circ \myfone \circ \mv{h}_0 \right) \\
  \myfthr \circ \myftwo \circ \myfone \circ \mv{h}_0 
      \end{matrix}
    \right]
  \end{equation}
  
  \begin{equation} \label{eq:generalizations-superdiagonal-M4-iteration5}
    \circ_{i=1}^{5}M_{ad}  
    \left(
      \begin{bmatrix}
          \mv{h}_0 \\
          0 \\
          0 \\
          0 \\
      \end{bmatrix}
      \right) = 
    \left[
      \begin{matrix}
  \mv{h}_0 \\
  \left(\myS \circ \myftwo \circ \myS \circ \myftwo \circ \myfone \circ \mv{h}_0 +  \myS \circ \myftwo \circ \myfone \circ \mv{h}_0 +  \myfone \circ \mv{h}_0 \right) \\
  \left(\myftwo \circ \myS \circ \myftwo \circ \myfone \circ \mv{h}_0 +  \myftwo \circ \myfone \circ \mv{h}_0 \right) \\
  \left(\myfthr \circ \myftwo \circ \myS \circ \myftwo \circ \myfone \circ \mv{h}_0 +  \myfthr \circ \myftwo \circ \myfone \circ \mv{h}_0 \right) 
      \end{matrix}
    \right]
  \end{equation}
  
  In general, after the $k$-th iteration, if $S$ and $f_{\theta_i}$ are linear, with $k$ odd and $k \ge 3$ we have

  \begin{equation} \label{eq:generalizations-superdiagonal-M4-iterationk-odd}
    \circ_{i=1}^{k} M_{ad}  
    \left(
      \begin{bmatrix}
          \mv{h}_0 \\
          0 \\
          0 \\
          0 \\
      \end{bmatrix}
      \right) = 
    \left[
      \begin{matrix}
  \mv{h}_0 \\
  ( \circ_{i=0}^{\frac{k-1}{2}} (\myS \circ \myftwo) ) \circ \myfone \circ \mv{h}_0 \\
  \myftwo \circ ( \circ_{i=0}^{\frac{k-3}{2}} (\myS \circ \myftwo) ) \circ \myfone \circ \mv{h}_0 \\
  \myfthr \circ \myftwo \circ ( \circ_{i=0}^{\frac{k-3}{2}} (\myS \circ \myftwo) ) \circ \myfone \circ \mv{h}_0 
      \end{matrix}
    \right]
  \end{equation}

After the $k$-th iteration, if $S$ and $f_{\theta_i}$ are linear, with $k$ even and $k \ge 4$ we have

  \begin{equation} \label{eq:generalizations-superdiagonal-M4-iterationk-even}
    \circ_{i=1}^{k} M_{ad}  
    \left(
      \begin{bmatrix}
          \mv{h}_0 \\
          0 \\
          0 \\
          0 \\
      \end{bmatrix}
      \right) = 
    \left[
      \begin{matrix}
  \mv{h}_0 \\
  ( \circ_{i=0}^{\frac{k-3}{2}} (\myS \circ \myftwo) ) \circ \myfone \circ \mv{h}_0 \\
  \myftwo \circ ( \circ_{i=0}^{\frac{k-3}{2}} (\myS \circ \myftwo) ) \circ \myfone \circ \mv{h}_0 \\
  \myfthr \circ \myftwo \circ ( \circ_{i=0}^{\frac{k-4}{2}} (\myS \circ \myftwo) ) \circ \myfone \circ \mv{h}_0 
      \end{matrix}
    \right]
  \end{equation}

So, in the liner case, the convergence of the above is determined by the convergence of the infinite product of $S \circ \myftwo$ alone!  Note, here $\myftwo$, and the $f_{\theta_j}$, are generally non-linear functions and the power-series is not available in closed form.  However, perhaps special cases of $f_{\theta_j}$ can be considered.

% \subsection{Top row of zeros} \label{sec:generalizations-RNN}

% Assigning zero blocks to the top row recalls the RNN \eqref{eq:RNN-dyamics}, i.e, 
% % Full matrix
% \begin{equation} \label{eq:generalizations-RNN}
%     \begin{bmatrix}
%         0 & 0  & 0  & 0  & 0 \\
%         \Wg{W_{2,1}} & \Wy{W_{2,2}}  & \Wr{W_{2,3}}  & \Wr{W_{2,4}}  & \Wr{W_{2,5}} \\
%         \Wb{W_{3,1}} & \Wg{W_{3,2}}  & \Wy{W_{3,3}}  & \Wr{W_{3,4}}  & \Wr{W_{3,5}} \\
%         \Wb{W_{4,1}} & \Wb{W_{4,2}}  & \Wg{W_{4,3}}  & \Wy{W_{4,4}}  & \Wr{W_{4,5}} \\
%         \Wb{W_{5,1}} & \Wb{W_{5,2}}  & \Wb{W_{5,3}}  & \Wg{W_{5,4}}  & \Wy{W_{5,5}} \\
%     \end{bmatrix}
%     =
%     \begin{bmatrix}
%         0 & 0 \\
%         W_1 & W_2 \\
%     \end{bmatrix}
% \end{equation}
% which is an RNN.





==> sections/old/Outtakes/MLP.tex <==
%\emph{Note the striking resemblance between the RNN iteration in \eqref{eq:rnn} and the MLP feed forward network in \eqref{eqn:nestedfx}.}  It is precisely this resemblance which inspires our work.   In particular, we will show that MLP feed forward network in \eqref{eqn:nestedfx} can be viewed as a special case of the the RNN iteration in \eqref{eq:rnn}.  




%Consider the following iterative map, similar to that found in \eqref{eq:blockwise}.

% \section{CNNs, RNNs and MLPs as iterative networks} \label{sec:RNN_iterative}

% Wikipedia states...
% \begin{quotation}
%     The term ``recurrent neural network" is used to refer to the class of networks with an infinite impulse response, whereas ``convolutional neural network'' refers to the class of finite impulse response. Both classes of networks exhibit temporal dynamic behavior.\cite{miljanovic2012comparative} A finite impulse recurrent network is a directed acyclic graph that can be unrolled and replaced with a strictly feedforward neural network, while an infinite impulse recurrent network is a directed cyclic graph that can not be unrolled.    
% \end{quotation}

% Let the columns $X$ be sequential data $X=[x_0, x_1, x_2, \dots x_N]$ and define the block non-linear function





%The map $M$ is a fixed autonomous discrete dynamical system, exactly like the RNN in \eqref{eq:RNN_defn}, except that its function form is \emph{sparse}.  Further, since the fixed point of $M$ \eqref{eq:MLP_fixed_point} is independent of the input $\mv{x}$, the map $M$ is a finite impulse response (FIR) dynamical system with respect to the input $\mv{x}$.

%Any MLP can be written as a block non-linear function as in \eqref{eq:MLP_blockwise_sparse} by adding more rows to $M$, one for each layer of the MLP. The map $M$ is a fixed map that is iterated just as the RNN map in \eqref{eq:RNN_defn}, but only a \emph{subset}  of its output is identical to the MLP in \eqref{eqn:MLP_nested_3}.  Maps such as $M$ blur the distinction between these two classes of neural networks as \emph{both MLPs and RNNs are a special case of iterated block non-linear functions}. %Thus we claim $M$ is both a RNN and a MLP.

%One can see from \eqref{eqn:toomanyiterations} that $M$ is a dynamical systems with some interesting properties.



==> sections/old/Outtakes/Numerical_experiments.tex <==

%Experiments were conducted across several areas of focus.  Initial efforts using the iterative network architecture were focused on determining the guiding principles associated with the location and arrangement of trainable parameters within the weight space as detailed in Section \ref{sec:results_model_structure}.  Additionally, general comparisons were conducted in which INN performance was benchmarked against LSTM models with comparable numbers of trainable weights using the sequential anomaly detection problems in Section \ref{sec:results_model_comparisons}. 
%Incorporating both sets of findings, further rounds of experiments were conducted exploring the use and benefits of sparsely arranged parameters within the weight space.  The concept of sparsely parameterized neural networks is explored from several angles in Section \ref{sec:results_density_sparsity}.  Initially, sparsity is examined in instances with number of trainable parameters left to vary while weight matrix dimensions remain fixed as in Section \ref{sec:results_density}.  Then, the effects of sparsity are explored with the number of trainable parameters fixed and matrix dimensions left to vary in Section \ref{sec:results_sparsity}.  




%\subsection{Sequential anomaly detection} \label{sec:numerical_experiment_sequential_anomaly}

%An anomaly detection task was created using sequential data sets and referred to as randomized anomaly detection. In this problem, the task of each sequence is to select which image is unlike the others and provide its indexed location after processing each sequence.  

%\subsubsection{Sequential transformations} \label{sec:numerical_experiment_sequential_transformations}

%In the case of anomaly detection sequences in which transforms may be used to generate anomalies, the effects applied to the image are varied among several predefined combinations of transformations.  In these cases, it is somewhat counter intuitive in that anomalies with less severe transformations are typically harder to identify than anomalies with greater applied distortions.  This inverse relationship between severity of transformations and problem difficulty runs contrary to typical classification problems in which applying stronger transforms often raises the problem difficulty.  With this in mind, the transformations used in anomaly detection sequences were generally softened with the objective of creating a problem set that would pose a sufficient challenge to differentiate performance across several architectures.  The combinations of transformations which were utilized in these sequential anomaly detection problems are outlined below.

%\begin{figure}[htbp]
%     \centering
%     \begin{minipage}[b]{0.5\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{Figures/mnist_baseline.png}
%         \label{fig:mnistbaselineanomaly}
%     \end{minipage}
%     \hfill
%     \begin{minipage}[b]{0.5\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{Figures/mnist_perspective_small_anomaly.png}
%         \label{fig:mnistperspectivesmallanomaly}
%     \end{minipage}
%     \hfill
%     \begin{minipage}[b]{0.5\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{Figures/mnist_perspective_anomaly.png}
%         \label{fig:mnistperspectiveanomaly}
%     \end{minipage}
%     \hfill
%     \begin{minipage}[b]{0.5\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{Figures/mnist_erase_anomaly.png}
%         \label{fig:mnisteraseanomaly}
%     \end{minipage}
%     \hfill
%     \begin{minipage}[b]{0.5\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{Figures/mnist_noise_anomaly.png}
%         \label{fig:mnistnoiseanomaly}
%     \end{minipage}
%     \hfill
%     \begin{minipage}[b]{0.5\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{Figures/mnist_both_anomaly.png}
%         \label{fig:mnistbothanomaly}
%     \end{minipage}
%     \hfill
%     \begin{minipage}[b]{0.5\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{Figures/mnist_blur_anomaly.png}
%         \label{fig:mnistbluranomaly}
%     \end{minipage}
%     \hfill
%     \begin{minipage}[b]{0.5\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{Figures/mnist_sharpness_anomaly.png}
%         \label{fig:mnistsharpnessanomaly}
%     \end{minipage}
%        \caption{The samples above from the MNIST data set are used to demonstrate the various combinations of transformations used in sequential data sets for anomaly detection with all transforms being resized and normalized as in (a).  In addition to being resized and normalized (a), other examples include small random pespective (b), random perspective (c), erase (d), noise (e), erase and perspective (f) and blur (g). One of the above transformations is selected and applied to a series of data while another transformation is applied to the randomly assigned outlier.}
%        \label{fig:sequential_transformations}
%\end{figure}

%\medskip
%\textbf{Baseline}
%\begin{itemize}
%    \item Resized $X\in\mathbb{R}_{50 \times 50}$
%    \item Normalized distribution $X \sim \mathcal{N} (0.1307, 0.3081)$
%\end{itemize}

%\textbf{Perspective Small}
%\begin{itemize}
%    \item Resized $X\in\mathbb{R}_{50 \times 50}$
%    \item Random perspective with default distortion scale of 0.5
%    \item Normalized distribution $X \sim \mathcal{N} (0.1307, 0.3081)$
%\end{itemize}

%\textbf{Perspective}
%\begin{itemize}
%    \item Resized $X\in\mathbb{R}_{50 \times 50}$
%    \item Random perspective with default distortion scale increased to 0.9
%    \item Normalized distribution $X \sim \mathcal{N} (0.1307, 0.3081)$
%\end{itemize}

%\textbf{Erase}
%\begin{itemize}
%    \item Resized $X\in\mathbb{R}_{50 \times 50}$
%    \item Random erasing with proportion of erased area to range between (0.1, 0.2)
%    \item Normalized distribution $X \sim \mathcal{N} (0.1307, 0.3081)$
%\end{itemize}

%\textbf{Noise}
%\begin{itemize}
%    \item Resized $X\in\mathbb{R}_{50 \times 50}$
%    \item Gaussian noise applied with a standard deviation of 0.01
%    \item Normalized distribution $X \sim \mathcal{N} (0.1307, 0.3081)$
%\end{itemize}

%\textbf{Erasing \& Perspective}
%\begin{itemize}
%    \item Resized $X\in\mathbb{R}_{50 \times 50}$
%    \item Random erasing with proportion of erased area to range between (0.1, 0.2)
%    \item Random perspective with default distortion scale increased to 0.9
%    \item Normalized distribution $X \sim \mathcal{N} (0.1307, 0.3081)$
%\end{itemize}

%\textbf{Blur}
%\begin{itemize}
%    \item Resized $X\in\mathbb{R}_{50 \times 50}$
%    \item Gaussian blur applied with kernel size 15
%    \item Normalized distribution $X \sim \mathcal{N} (0.1307, 0.3081)$
%\end{itemize}

%\textbf{Sharpness}
%\begin{itemize}
%    \item Resized $X\in\mathbb{R}_{50 \times 50}$
%    \item Randomly adjusted sharpness with a factor of 4
%    \item Normalized distribution $X \sim \mathcal{N} (0.1307, 0.3081)$
%\end{itemize}

%\subsection{Random anomaly detection} \label{sec:numerical_experiment_random_anomaly}

%The random anomaly detection data set represents a much more challenging problem than the classification task.  Within a given sequence of length N, all of the nonanomalous images will have the same randomly selected combination of random transformations from Fig. \ref{fig:sequential_transformations} applied while the other will have a different randomly selected combination of random transformations applied.  In this case for example, N-1 different examples of a handwritten number are selected from the MNIST data set and given the same randomly selected combination of random transformations while another different example of the same handwritten number is given a different combination of random transformations.  Aside from each copy of the images being different at the onset, each of the transformations may be applied differently.  For instance, each randomly cropped, oriented or shifted image would have the transformation applied differently in a randomized way, yet would not be considered anomalous while the other randomly selected example with its own set of transforms would be the anomaly.  A series of examples of the random anomaly detection data set with sequence length 9 is provided below.  Each step of the sequence contains a binary ground truth value indicating whether that step is the anomaly.  At the end of the sequence, the last blank image is paired with the ground truth index location of the anomaly and indicates the algorithm should provide its estimate.  Further increasing the length of this data set appears to increase the challenge in terms of memory and problem complexity while reducing certainty by way of more competing options.

%\begin{figure}[htbp]
%     \centering
%     \includegraphics[width=0.5\textwidth]{Figures/randomanomaly.png}
%     \caption{Examples of multiple series from the random anomaly detection data set with sequence length set to nine. Each series is presented horizontally with the anomaly outlined by a light grey square.}
%     \label{fig:randomanomaly2}
%\end{figure}

==> sections/old/Outtakes/RNN.tex <==
% It has been noted that 

% \begin{quotation}
%     The term "recurrent neural network" is used to refer to the class of networks with an infinite impulse response, whereas "convolutional neural network" refers to the class of finite impulse response. Both classes of networks exhibit temporal dynamic behavior. A finite impulse recurrent network is a directed acyclic graph that can be unrolled and replaced with a strictly feedforward neural network, while an infinite impulse recurrent network is a directed cyclic graph that can not be unrolled. \footnote{https://en.wikipedia.org/wiki/Recurrent\_neural\_network}
% \end{quotation}

% \noindent and     






==> sections/old/Outtakes/continuation.tex <==
%So, what is $M_{\infty}$?  Is it an RNN or an MLP?  Or is it something else?  In particular, any MLP (or any sequential NN what-so-ever) with finite impulse response can be written as a dynamical system with infinite impulse response.  Does that lead to anything interesting?  Or is it just a mathematical curiosity?  Just wait and see! \todo{Needs better text :-)}  

==> sections/old/Outtakes/generalizations.tex <==

% % Above the diagonal
% For example
% \begin{equation}
% \begin{aligned}
%     &\begin{bmatrix}
%         \Wy{I}   & \Wr{H_0}  & 0      & 0 \\
%         \Wg{f_{\theta_1}} & 0         & 0      & 0 \\
%         0         & \Wg{f_{\theta_2}} & 0      & 0 \\
%         \Wb{S}   & 0         & \Wg{f_{\theta_3}} & 0 \\
%     \end{bmatrix}
%     \circ 
%    \begin{bmatrix}
%         \Wy{I}   & \Wr{H_0}  & 0      & 0 \\
%         \Wg{f_{\theta_1}} & 0         & 0      & 0 \\
%         0         & \Wg{f_{\theta_2}} & 0      & 0 \\
%         \Wb{S}   & 0         & \Wg{f_{\theta_3}} & 0 \\
%     \end{bmatrix}
%     \circ
%     \begin{bmatrix}
%         \Wy{I}   & \Wr{H_0}  & 0      & 0 \\
%         \Wg{f_{\theta_1}} & 0         & 0      & 0 \\
%         0         & \Wg{f_{\theta_2}} & 0      & 0 \\
%         \Wb{S}   & 0         & \Wg{f_{\theta_3}} & 0 \\
%     \end{bmatrix}
%         \circ
%     \begin{bmatrix}
%         X \\
%         0 \\
%         0 \\
%         0 \\
%     \end{bmatrix} 
%     = \\ \\
%     & \hspace{1cm}
%     \begin{bmatrix}
%         X + 2 H_0(f_{\theta_1}(X)) \\
%         f_{\theta_1}(X) + f_{\theta_1}(H_0(f_{\theta_1}(X))) \\
%         f_{\theta_2}(f_{\theta_1}(X)) \\
%         S(X) +S(H_0(f_{\theta_1}(X))) + f_{\theta_3}(f_{\theta_2}(f_{\theta_1}(X))) \\
%     \end{bmatrix} 
%     \label{eqn:skipiterationcolor}
% \end{aligned}
% \end{equation}

% This is not a fixed point. Discuss sparsity


==> sections/old/Outtakes/introduction.tex <==
%In particular, disparate models, such as MLPs and RNNs, actually lie on a continuum. For example, there are \emph{sparse} RNNs that are exactly equivalent to MLPs, and there are \emph{dense} MLPs that become recurrent when armed with a single additional parameter.  Such NNs are really two-sides of the same coin.  In fact, sparse RNNs, and more general models derived from them, will form the focus of our work.  Of course, sparsity is a well-known technique for improving the efficiency, stability, and effectiveness of neural networks \cite{FIXME}.  However, in this text we explore how the manner in which an RNN is sparsified can have a significant impact on the resulting model.  For example, it is possible that a sparse "RNN" may not actually be recurrent at all, either by chance or by design.  Accordingly, we introduce the idea of an Iterative Neural Network (INN) \ref{defn_block_iterative_map} to emphasize that the sparsification of an RNN can lead to a variety of different models, some of which are not recurrent, but all of which are iterative.  In fact, many common neural network models can be embedded into an iterative map, and studying the iterative version of common neural networks can provide valuable insights into those models. By understanding the relationship between these models, we can gain a deeper understanding of the underlying principles of neural networks and how to improve their performance.

%In section \ref{sec:method_mlp}, we remind the reader of several fundamental neural network architectures which are later used to explore performance across various problem sets.  The iterative nature of Recurrent Neural Network (RNN) architectures is also discussed as a generalized neural network architecture with several reflections in dynamical systems theory \cite{https://doi.org/10.48550/arxiv.1801.01078, _1998}.  Moreover, we show how traditional feed-forward multi-layer perception networks may be represented by RNNs as a special case implemented through constraints regarding the arrangement of trainable weights.  An overview is provided of the standard long short-term memory (LSTM) network \cite{10.1162/neco_a_01199} as a common architecture deployed over sequential data sets and therefore a natural choice for performance benchmarking \cite{https://doi.org/10.48550/arxiv.1508.02774}.


==> sections/old/Sequential2D_old.tex <==
\subsection{The general sequential2D map} \label{sec:generalizations}
This opens an entire range of new possibilities when considering a block iterative function of the form

% Full matrix
\begin{equation} \label{eq:GEN_all}
    \begin{bmatrix}
        \Wy{W_{1,1}} & \Wr{W_{1,2}}  & \Wr{W_{1,3}}  & \Wr{W_{1,4}}  & \Wr{W_{1,5}} \\
        \Wg{W_{2,1}} & \Wy{W_{2,2}}  & \Wr{W_{2,3}}  & \Wr{W_{2,4}}  & \Wr{W_{2,5}} \\
        \Wb{W_{3,1}} & \Wg{W_{3,2}}  & \Wy{W_{3,3}}  & \Wr{W_{3,4}}  & \Wr{W_{3,5}} \\
        \Wb{W_{4,1}} & \Wb{W_{4,2}}  & \Wg{W_{4,3}}  & \Wy{W_{4,4}}  & \Wr{W_{4,5}} \\
        \Wb{W_{5,1}} & \Wb{W_{5,2}}  & \Wb{W_{5,3}}  & \Wg{W_{5,4}}  & \Wy{W_{5,5}} \\
    \end{bmatrix}
\end{equation}

In this notation, 
\begin{itemize}
\item $\Wg{W_{i+1,i}}$ corresponds to a standard MLP or, more generally, an NN that can be implemented as a Pytorch or Keras Sequential container.
\item $\Wb{W_{i+k,i}}, \; k>1$ corresponds to skip connections and finite impulse response (FIR) filters.
%\item We began the exploration of $\Wy{W_{i,i}}$ with the introduction of the $I$ in \eqref{FIXME} corresponds infinite impulse response filters.
%\item What do $\Wr{W_{i,j}}, \; j>i$ correspond to?  They are actually \emph{feedback} connections which also lead to infinite impulse response filters and classic RNNs.
\end{itemize}

\subsubsection{Diagonal blocks} \label{sec:generalization_diagonal}

\begin{equation}
M_d = 
  \left[
      \begin{matrix}
  \Wy{I} & 0 & 0 & 0\\
  \myfone & \Wy{S} & 0 & 0\\
  0 & \myftwo & 0 & 0\\
  0 & 0 & \myfthr & 0
      \end{matrix}
    \right]
  \end{equation}
  
  \begin{equation}
    \circ_{i=1}^3 M_{d}  
    \left(
      \begin{bmatrix}
          \mv{x} \\
          0 \\
          0 \\
          0 \\
      \end{bmatrix}
      \right) = 
    \left[
      \begin{matrix}
  \mv{x} \\
  \left(\Wy{S} \circ \myfone \circ \mv{x} +  \Wy{S} \circ \Wy{S} \circ \myfone \circ \mv{x} +  \myfone \circ \mv{x} \right) \\
  \left(\myftwo \circ \Wy{S} \circ \myfone \circ \mv{x} +  \myftwo \circ \myfone \circ \mv{x} \right) \\
  \myfthr \circ \myftwo \circ \myfone \circ \mv{x} 
      \end{matrix}
    \right]
  \end{equation}
  
  \begin{equation}
    \circ_{i=1}^4 M_{d}  
    \left(
      \begin{bmatrix}
          \mv{x} \\
          0 \\
          0 \\
          0 \\
      \end{bmatrix}
      \right) = 
    \left[
      \begin{matrix}
  \mv{x} \\
  \left(\Wy{S} \circ \myfone \circ \mv{x} +  \Wy{S} \circ \Wy{S} \circ \myfone \circ \mv{x} +  \Wy{S} \circ \Wy{S} \circ \Wy{S} \circ \myfone \circ \mv{x} +  \myfone \circ \mv{x} \right) \\
  \left(\myftwo \circ \Wy{S} \circ \myfone \circ \mv{x} +  \myftwo \circ \Wy{S} \circ \Wy{S} \circ \myfone \circ \mv{x} +  \myftwo \circ \myfone \circ \mv{x} \right) \\
  \left(\myfthr \circ \myftwo \circ \Wy{S} \circ \myfone \circ \mv{x} +  \myfthr \circ \myftwo \circ \myfone \circ \mv{x} \right) 
      \end{matrix}
    \right]
  \end{equation}

  In general, after the $k$-th iteration, if $S$ and $f_{\theta_i}$ are linear, with $k \ge 3$ we have

  \begin{equation}
    \circ_{i=1}^k M_{d}  
    \left(
      \begin{bmatrix}
          \mv{x} \\
          0 \\
          0 \\
          0 \\
      \end{bmatrix}
      \right) = 
    \left[
      \begin{matrix}
  \mv{x} \\
  ( \circ_{i=0}^{k-1} \Wy{S} ) \circ \myfone \circ \mv{x} \\
  \myftwo \circ ( \circ_{i=0}^{k-2} \Wy{S} ) \circ \myfone \circ \mv{x} \\
  \myfthr \circ \myftwo \circ ( \circ_{i=0}^{k-3} \Wy{S} ) \circ \myfone \circ \mv{x} 
      \end{matrix}
    \right]
  \end{equation}

So, in the linear case, the convergence of the above is determined by the convergence of the infinite product of $S$ alone!  I.e., if we choose $S$ \emph{and} the $f{\theta_i}$ to be a linear function  where the power-series is well understood.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Super-diagonal blocks} \label{sec:generalization_superdiagonal}

\begin{equation}
  M_{ad} = 
    \left[
      \begin{matrix}
  \myI & 0 & 0 & 0\\
  \myfone & 0 & \myS & 0\\
  0 & \myftwo & 0 & 0\\
  0 & 0 & \myfthr & 0
      \end{matrix}
    \right]
  \end{equation}
  
  \begin{equation}
    \circ_{i=1}^{3}M_{ad}  
    \left(
      \begin{bmatrix}
          \mv{x} \\
          0 \\
          0 \\
          0 \\
      \end{bmatrix}
      \right) = 
      \left[
      \begin{matrix}
  \mv{x} \\
  \left(\myS \circ \myftwo \circ \myfone \circ \mv{x} +  \myfone \circ \mv{x} \right) \\
  \myftwo \circ \myfone \circ \mv{x} \\
  \myfthr \circ \myftwo \circ \myfone \circ \mv{x} 
      \end{matrix}
    \right]
  \end{equation}
  
  \begin{equation}
    \circ_{i=1}^{4}M_{ad}  
    \left(
      \begin{bmatrix}
          \mv{x} \\
          0 \\
          0 \\
          0 \\
      \end{bmatrix}
      \right) = 
    \left[
      \begin{matrix}
  \mv{x} \\
  \left(\myS \circ \myftwo \circ \myfone \circ \mv{x} +  \myfone \circ \mv{x} \right) \\
  \left(\myftwo \circ \myS \circ \myftwo \circ \myfone \circ \mv{x} +  \myftwo \circ \myfone \circ \mv{x} \right) \\
  \myfthr \circ \myftwo \circ \myfone \circ \mv{x} 
      \end{matrix}
    \right]
  \end{equation}
  
  \begin{equation}
    \circ_{i=1}^{5}M_{ad}  
    \left(
      \begin{bmatrix}
          \mv{x} \\
          0 \\
          0 \\
          0 \\
      \end{bmatrix}
      \right) = 
    \left[
      \begin{matrix}
  \mv{x} \\
  \left(\myS \circ \myftwo \circ \myS \circ \myftwo \circ \myfone \circ \mv{x} +  \myS \circ \myftwo \circ \myfone \circ \mv{x} +  \myfone \circ \mv{x} \right) \\
  \left(\myftwo \circ \myS \circ \myftwo \circ \myfone \circ \mv{x} +  \myftwo \circ \myfone \circ \mv{x} \right) \\
  \left(\myfthr \circ \myftwo \circ \myS \circ \myftwo \circ \myfone \circ \mv{x} +  \myfthr \circ \myftwo \circ \myfone \circ \mv{x} \right) 
      \end{matrix}
    \right]
  \end{equation}
  
  In general, after the $k$-th iteration, if $S$ and $f_{\theta_i}$ are linear, with $k$ odd and $k \ge 3$ we have

  \begin{equation}
    \circ_{i=1}^{k} M_{ad}  
    \left(
      \begin{bmatrix}
          \mv{x} \\
          0 \\
          0 \\
          0 \\
      \end{bmatrix}
      \right) = 
    \left[
      \begin{matrix}
  \mv{x} \\
  ( \circ_{i=0}^{\frac{k-1}{2}} (\myS \circ \myftwo) ) \circ \myfone \circ \mv{x} \\
  \myftwo \circ ( \circ_{i=0}^{\frac{k-3}{2}} (\myS \circ \myftwo) ) \circ \myfone \circ \mv{x} \\
  \myfthr \circ \myftwo \circ ( \circ_{i=0}^{\frac{k-3}{2}} (\myS \circ \myftwo) ) \circ \myfone \circ \mv{x} 
      \end{matrix}
    \right]
  \end{equation}

After the $k$-th iteration, if $S$ and $f_{\theta_i}$ are linear, with $k$ even and $k \ge 4$ we have

  \begin{equation}
    \circ_{i=1}^{k} M_{ad}  
    \left(
      \begin{bmatrix}
          \mv{x} \\
          0 \\
          0 \\
          0 \\
      \end{bmatrix}
      \right) = 
    \left[
      \begin{matrix}
  \mv{x} \\
  ( \circ_{i=0}^{\frac{k-3}{2}} (\myS \circ \myftwo) ) \circ \myfone \circ \mv{x} \\
  \myftwo \circ ( \circ_{i=0}^{\frac{k-3}{2}} (\myS \circ \myftwo) ) \circ \myfone \circ \mv{x} \\
  \myfthr \circ \myftwo \circ ( \circ_{i=0}^{\frac{k-4}{2}} (\myS \circ \myftwo) ) \circ \myfone \circ \mv{x} 
      \end{matrix}
    \right]
  \end{equation}

So, in the liner case, the convergence of the above is determined by the convergence of the infinite product of $S \circ \myftwo$ alone!  Note, here $\myftwo$, and the $f_{\theta_i}$, are generally non-linear functions and the power-series is not available in closed form.  However, perhaps special cases of $f_{\theta_i}$ can be considered.

\subsubsection{Top row of zeros} \label{sec:generalization_RNN}

Assigning zero blocks to the top row recalls the RNN \eqref{eq:RNN_DS_RHS}, i.e, 
% Full matrix
\begin{equation}
    \begin{bmatrix}
        0 & 0  & 0  & 0  & 0 \\
        \Wg{W_{2,1}} & \Wy{W_{2,2}}  & \Wr{W_{2,3}}  & \Wr{W_{2,4}}  & \Wr{W_{2,5}} \\
        \Wb{W_{3,1}} & \Wg{W_{3,2}}  & \Wy{W_{3,3}}  & \Wr{W_{3,4}}  & \Wr{W_{3,5}} \\
        \Wb{W_{4,1}} & \Wb{W_{4,2}}  & \Wg{W_{4,3}}  & \Wy{W_{4,4}}  & \Wr{W_{4,5}} \\
        \Wb{W_{5,1}} & \Wb{W_{5,2}}  & \Wb{W_{5,3}}  & \Wg{W_{5,4}}  & \Wy{W_{5,5}} \\
    \end{bmatrix}
    =
    \begin{bmatrix}
        0 & 0 \\
        W_1 & W_2 \\
    \end{bmatrix}
\end{equation}
which is an RNN.


% % Above the diagonal
% For example
% \begin{equation}
% \begin{aligned}
%     &\begin{bmatrix}
%         \Wy{I}   & \Wr{H_0}  & 0      & 0 \\
%         \Wg{f_{\theta_1}} & 0         & 0      & 0 \\
%         0         & \Wg{f_{\theta_2}} & 0      & 0 \\
%         \Wb{S}   & 0         & \Wg{f_{\theta_3}} & 0 \\
%     \end{bmatrix}
%     \circ 
%    \begin{bmatrix}
%         \Wy{I}   & \Wr{H_0}  & 0      & 0 \\
%         \Wg{f_{\theta_1}} & 0         & 0      & 0 \\
%         0         & \Wg{f_{\theta_2}} & 0      & 0 \\
%         \Wb{S}   & 0         & \Wg{f_{\theta_3}} & 0 \\
%     \end{bmatrix}
%     \circ
%     \begin{bmatrix}
%         \Wy{I}   & \Wr{H_0}  & 0      & 0 \\
%         \Wg{f_{\theta_1}} & 0         & 0      & 0 \\
%         0         & \Wg{f_{\theta_2}} & 0      & 0 \\
%         \Wb{S}   & 0         & \Wg{f_{\theta_3}} & 0 \\
%     \end{bmatrix}
%         \circ
%     \begin{bmatrix}
%         X \\
%         0 \\
%         0 \\
%         0 \\
%     \end{bmatrix} 
%     = \\ \\
%     & \hspace{1cm}
%     \begin{bmatrix}
%         X + 2 H_0(f_{\theta_1}(X)) \\
%         f_{\theta_1}(X) + f_{\theta_1}(H_0(f_{\theta_1}(X))) \\
%         f_{\theta_2}(f_{\theta_1}(X)) \\
%         S(X) +S(H_0(f_{\theta_1}(X))) + f_{\theta_3}(f_{\theta_2}(f_{\theta_1}(X))) \\
%     \end{bmatrix} 
%     \label{eqn:skipiterationcolor}
% \end{aligned}
% \end{equation}

% This is not a fixed point. Discuss sparsity


\subsection{Sequential2D vs Sequential1D}

\todo{This section is copied from the ICMLA paper and needs to be rewritten}

*****COPIED FROM OTHER PAPER, NEEDS TO BE REWRITTEN*****

*****COPIED FROM OTHER PAPER, NEEDS TO BE REWRITTEN*****

*****COPIED FROM OTHER PAPER, NEEDS TO BE REWRITTEN*****


Sequential2D refers to the 2D matrix of functions, as opposed to the 1D array of functions in a Pytorch or Keras Sequential container.  Specifically, Sequential2D is a PyTorch module that allows one to define a neural network by specifying a sequence of layers. The layers are defined as a list of PyTorch modules, which can be any type of layer or operation supported by PyTorch \cite{pytorch2017automatic}. Theoretically Sequential2D  can be used with a variety of neural network models(nn.Modules) \cite{pytorch2017automatic}, including MLPs, RNNs, LSTMs, attention, transformers, and convolutional neural networks. However, our prime focus in this paper is on attention blocks \cite{radford2019gpt2} used in GPT-2.  

Of course, we are not the first to propose thinking about NNs in terms of a block matrix structure. For example, the work by\cite{narang2017blocksparse} provides a promising approach for reducing the size and computational complexity of RNNs without sacrificing accuracy. Their block-sparse RNNs could be used to make RNNs more accessible to a wider range of applications, and could also be used to improve the performance of RNNs on existing applications. Further, in \cite{narang2017blocksparse} the authors observe that block sparsity is a more structured form of sparsity than unstructured sparsity\footnote{Structured sparsity refers to a specific pattern of zeros in a sparse matrix, while unstructured sparsity lacks any regularity in the distribution of zeros. Block sparsity is a form of structured sparsity where zeros appear in contiguous blocks.}, and can lead to better performance on hardware architectures that support block-sparse matrix multiplication. There are few points we wish to emphasize on:
\begin{itemize}
     
    \item As can be seen in (\ref{eq:long-eq}) there is additional information propagation in a Sequential2D that is not possible in a standard Sequential container.  For example, the output $Y$ depends on $f_{m,0}(X) + f_{m,1}(H) + \hdots + f_{m,n}(Y)$ and not just $f_{m,n-1}(H_k)$ and it is precisely such information propagation that is required for SC.
    \item As we will demonstrate in the next section, a Sequential2D neural network can be thought of as an RNN, in that a fixed Sequential2D is iterated across a given data set.      

    \item \emph{We propose Sequential2D as an enhanced orchestrator which provides insights into not only the width and depth of the network but two more scenarios: (1) intra-connections for a model such as a skip connection and (2) inter-connections between two or more models.}\footnote{Note inter-connections is not the focus of this paper and are left for future work.}
    % and understanding the iterative structure of a Sequential2D is important for understanding the applications of Sequential2D.  In particular, in the next section we will demonstrate a close connection between Sequential2D, RNNs, and SC.
\end{itemize}

